A new classification of links and some calculations using it

A new classification theorem for links by the authors and Roger Fenn leads to computable link invariants. As an illustration we distinguish the left and right trefoils and recover the result of Carter et al that the 2-twist-spun trefoil is not isotopic to its orientation reverse. We sketch the proof the classification theorem. Full details will appear elsewhere

==> maple/homology <==

# homology

# If A and B are matrices such that A*B=0 then homology(B,A) will
# compute ker(A)/im(B), i.e. it will compute the torsion coefficients,
# the rank and a set of generators. `normformnew` is a package which
# includes `ismithex` and should be read in first.


homology:=proc(B,A)
local m,k,S1,S2,L1,L2,R1,R2,r,C,R1inv,L,tors,gen,i;
  k:=linalg[coldim](A);
  m:=linalg[coldim](B);
  S1:=ismithex(A,'L1','R1');
  r:=linalg[rank](S1);
  if r=k then                                    #
    print(`Homology is 0`);RETURN()              #  inserted
  else                                           #
    C:=linalg[submatrix](evalm(R1&*B),r+1..k,1..m);
    S2:=ismithex(C,'L2','R2');
    R1inv:=linalg[inverse](R1);
    L:=linalg[matrix](k,k,0);
    L:=linalg[copyinto](L2,L,r+1,1);
    L:=linalg[copyinto](linalg[matrix](r,r,1),L,1,k-r+1);
    L:=evalm(R1inv&*L);
    tors:=[];
    for i to k-r while S2[i,i]<>0 do
      if S2[i,i]<>1 then tors:=[op(tors),S2[i,i]] fi
    od;
    if i=k-r+1 then                              #
      print(`Homology is 0`);RETURN()            #  inserted
    else                                         #
      gen:=linalg[submatrix](L,1..k,i-nops(tors)..k-r);
      print(`Torsion coeffs`,tors,`Rank`,k-r-i+1,`Homology generators\
      are columns of`);
      print(gen)
    fi
  fi
end:



==> maple/normform <==

# normform: A PACKAGE FOR THE COMPUTATION OF SEVERAL MATRIX NORMAL FORMS
# ----------------------------------------------------------------------
# 
# This file contains six routines for the computation of normal forms of
# matrices. The routines are:
#  - frobenius
#  - ratjordan
#  - jordansymbolic
#  - jordan
#  - smithex
#  - ismithex
# For each routine a description of the algorithm is added and comments are
# inserted.
# For help see the on-line help facility so type one of these:
#  - ?frobenius
#  - ?ratjordan
#  - ?jordansymbolic
#  - ?jordan
#  - ?smithex
#  - ?ismithex
# 
# AUTHORS: T.M.L. Mulders, A.H.M. Levelt
#          Mathematics Department
#          University of Nijmegen.
# E-mail:  mulders@sci.kun.nl, ahml@sci.kun.nl
#
# January 1993

macro(gcdexgeneral=`normform/gcdexgeneral`,
      simplalgebraic=`normform/simplalgebraic`,
      simplcomplex=`normform/simplcomplex`,
      simplratfunc=`normform/simplratfunc`,
      simplrational=`normform/simplrational`,
      multiplegeneral=`normform/multiplegeneral`,
      Id=`normform/Id`,
      basis=`normform/basis`,
      companion_to_ratjordan=`normform/companion_to_ratjordan`,
      cyclic_to_frobenius=`normform/cyclic_to_frobenius`,
      cyclic_vectors=`normform/cyclic_vectors`,
      deg_sort=`normform/deg_sort`,
      find_companion=`normform/find_companion`,
      find_ratjblock=`normform/find_ratjblock`,
      frobenius_to_invfact=`normform/frobenius_to_invfact`,
      frobenius_to_ratjordan=`normform/frobenius_to_ratjordan`,
      frobeniusform=`normform/frobeniusform`,
      identitymatrix=`normform/identitymatrix`,
      inv=`normform/inv`,
      invariant_to_jordan=`normform/invariant_to_jordan`,
      invfact_to_frobenius=`normform/invfact_to_frobenius`,
      jordanform=`normform/jordanform`,
      jordansymbolicform=`normform/jordansymbolicform`,
      priminv_to_ratjordan=`normform/priminv_to_ratjordan`,
      make_ratj_block=`normform/make_ratj_block`,
      mysmith=`normform/mysmith`,
      plist_to_polycompanion=`normform/plist_to_polycompanion`,
      ratjordan_to_jordan=`normform/ratjordan_to_jordan`,
      ratjordan_to_priminv=`normform/ratjordan_to_priminv`,
      ratjordanform=`normform/ratjordanform`,
      uppersmith=`normform/uppersmith`,
      zero_matrix=`normform/zero_matrix`,
      factors=readlib(factors)):


help:=proc()
  `help/help/old`:=readlib('help'): # save old help file definition
  help:=proc()
        local n;
          if type([args],list(string)) then
            n:=cat(`help/text/`,args);
            if type(eval(n,2),specfunc(string,TEXT)) then
              RETURN(print(eval(n,2)));
            fi;
          fi;
          `help/help/old`(args)
        end:
  help(args)
end:


############################################################################
############################################################################
##
##          frobenius
##
###########################################################################
###########################################################################
# A Maple program for the computation of the Frobenius normal form of
# a matrix.
# Authors: T.M.L. Mulders, A.H.M. Levelt
#          Mathematics Department
#          University of Nijmegen.
# E-mail: mulders@sci.kun.nl, ahml@sci.kun.nl
#
# January 1993


# A matrix F is said to be in Frobenius normal form if F=diag(C1,C2,..,Ck)
# where Ci is the companion matrix associated with a polynomial pi and the
# polynomials pi satify the condition: pi divides p(i+1) for i=1..(k-1).
# If A is a square matrix over a field K, then there exist square matrices
# P and F over K such that F is in Frobenius normal form and
#               inverse(P)*A*P = F.
# The matrix F is called the Frobenius normal form of A and is uniquely
# determined by A.
#
# The function frobenius computes the Frobenius normal form F of a matrix A,
# the transformation matrix P and its inverse P^(-1).
# Specifically:
# - frobenius(A) or frobenius(A,K) will return the Frobenius normal form F
#   of A.
# - frobenius(A,'P') or frobenius(A,K,'P') will do the same as frobenius(A)
#   (resp. frobenius(A,K)) but now the transformation matrix is assigned to P.
# - frobenius(A,'P','Pinv') or frobenius(A,K,'P','Pinv')will do the same as
#   frobenius(A,'P') (resp. frobenius(A,K,'P')) but now also the inverse of
#   the transformation matrix is assigned to Pinv.
# Here K is a set of RootOf's and/or radicals defining an algebraic extension
# of Q(the rational numbers).
#
# Global description of the algorithm:
# For a given n by n matrix A over a field K, let L be the linear
# transformation of K^n induced by A. A polycyclic basis of K^n with
# respect to L is a basis of the following form:
# v1,L*v1,..,L^(d1-1)*v1,v2,L*v2,..,L^(d2-1)*v2,..,vr,L*vr,..,L^(dr-1)*vr
# such that v1,L*v1,..,L^(d1-1)*v1,..,vi,L*vi,..,L^(di-1)*vi,L^di*vi are
# linearly dependent for i=1..r.
# It is easy to see that the matrix B of L with respect to a polycyclic basis
# is of the form plist_to_polycompanion(plist,x), where plist is a list of
# monic elements of K[x] of strictly increasing degree (for a description of
# plist_to_polycompanion see below).
# The computation of a polycyclic basis of K^n and the transformation
# matrix from A to B is performed in the function cyclic_vectors.
# Next we view K^n as a K[x]-module via x*v=B*v. Suppose that
# B=plist_to_polycompanion(plist,x), where plist=[p1,..,pr] and degree(pi)=di.
# Let G be the r by r upper triangular matrix such that G[i,j] satisfies:
#  pj=G[1,j]+G[2,j]*x^d1+G[3,j]*x^d2+..+G[j,j]*x^d(j-1),
# where degree(G[j,j])=dj-d(j-1) and degree(G[i,j])<di-d(i-1) (d0=0).
# Let R be the K[x]-submodule of K[x]^r generated by the columns of G.
# Representants for the elements of the quotient module K[x]^r/R are the
# vectors [L1,L2,..,Lr] where degree(Li)<di-d(i-1). By taking the
# coefficients of the Li the quotient module is identified with K^n. The
# multiplication by x on the quotient module is identified with the
# multiplication by B on K^n.
# Next we compute the Smith normal form S of G. Say L*S*R=G. If R' is the
# K[x]-submodule of K[x]^r generated by the columns of S we get the following
# diagram:  
#            ~                 ~                 ~
#    K^n <------- K[x]^r/R' -------> K[x]^r/R -------> K^n
#                              L                 
#     |               |                  |              |
#     |               |                  |              |
#     |F              |x                 |x             |B
#     |               |                  |              |
#     |               |                  |              |
#    \ /             \ /                \ /            \ /
#            ~                 ~                 ~
#    K^n <------- K[x]^r/R' -------> K[x]^r/R -------> K^n
#                              L                
#
# Here F is in Frobenius normal form and thus it is the Frobenius normal
# form of B (and thus of A). The computation of the Smith normal form of G
# is performed in the function cyclic_to_frobenius.


frobenius:=proc(A)
local AA,n,i,j;

  if not type(A,'matrix') then
    AA:=evalm(A)
  else
    AA:=A
  fi;
  if not type(AA,'matrix'('anything','square')) then
    ERROR(`expecting a square matrix`)
  fi;

  n:=linalg[rowdim](AA);
  for i to n do
    for j to n do
      if type(AA[i,j],indexed) then
        ERROR(`Unassigned array elements`)
      fi
    od
  od;

  if nargs>1 and type(args[2],set) then
    if args[2] ={I} then
      SIMPLIFY:=simplcomplex;
      GCDEX:=gcdexgeneral;
      frobeniusform(AA,args[3..nargs])
    else
      SIMPLIFY:=simplalgebraic;
      GCDEX:=gcdexgeneral;
      frobeniusform(AA,args[3..nargs])
    fi
  else
    if type(AA,'matrix'('rational')) then
      SIMPLIFY:=simplrational;
      GCDEX:=gcdex;
      frobeniusform(AA,args[2..nargs])
    else
      SIMPLIFY:=simplratfunc;
      GCDEX:=gcdexgeneral;
      frobeniusform(AA,args[2..nargs])
    fi
  fi

end:

`normform/frobeniusform`:=proc(A,P,Pinv)
local x,plist,inv_fact,V,Vinv,T,Tinv;

  if nargs=1 then
    plist:=cyclic_vectors(A,x);
    inv_fact:=cyclic_to_frobenius(plist,x)
  elif nargs=2 then
    plist:=cyclic_vectors(A,x,'V');
    inv_fact:=cyclic_to_frobenius(plist,x,'T');
    P:=map(SIMPLIFY,evalm(V&*T))
  else
    plist:=cyclic_vectors(A,x,'V','Vinv');
    inv_fact:=cyclic_to_frobenius(plist,x,'T','Tinv');
    P:=map(SIMPLIFY,evalm(V&*T));
    Pinv:=map(SIMPLIFY,evalm(Tinv&*Vinv))
  fi;

  invfact_to_frobenius(inv_fact,x)

end:


# cyclic_vectors computes a polycyclic basis of K^n with respect to A.
# If this basis is (b1,..,bn)=
# (v1,A*v1,..,A^(d1-1)*v1,v2,A*v2,..,A^(d2-1)*v2,..,vr,A*vr,..,A^(dr-1)*vr)
# and a1*b1+..+a(d1+..+di)*b(d1+..+di)+A^di*vi=0 we set
# pi=a1+a2*x+..+a(d1+..+di)*x^(d1+..+di-1)+x^(d1+..+di).
# cyclic_vectors returns the list [p1,..,pr].
# The matrix of A on this basis (b1,..,bn) is
# plist_to_polycompanion([p1,..,pr],x).

`normform/cyclic_vectors`:=proc(A,x,V,Vinv)
local i,j,l,n,r,carrier,car,U,Uinv,S,u,v,s,lincomb,plist,c,temp;

  n:=linalg[rowdim](A);
  U:=array(1..n,1..n);
  S:=array(1..n,1..n);
  plist:=[];
  if nargs>=3 then
    V:=array(1..n,1..n)
  fi;
  if nargs=4 then
    Vinv:=array(1..n,1..n)
  fi;

  carrier:=array(1..n);
  for i to n do carrier[i]:=0 od;
  lincomb:=array(1..n);

  r:=0;   # number of elements of basis already computed
  while r<n do
#######
# Start new cycle
#######
    for i to n while carrier[i]<>0 do od;   # find first gap
    v:=basis(n,i);
#######
    do
      u:=copy(v);
      for i to n do lincomb[i]:=0 od;

      # always v=u+U*lincomb
      for i to n do
        car:=carrier[i];
        if car<>0 and u[i]<>0 then
          c:=SIMPLIFY(u[i]/U[i,car]);
          u[i]:=0;
          for j from i+1 to n do u[j]:=SIMPLIFY(u[j]-c*U[j,car]) od;
          lincomb[car]:=c  
        fi
      od;

      i:=1;
      while i<=n and u[i]=0 do i:=i+1 od;
      if i<=n then
        # new element of basis
        r:=r+1;  
        carrier[i]:=r;   # this basis-element carries coordinate i

        #always U=V*S
        for j from i to n do U[j,r]:=u[j] od;
        if nargs>=3 then
          for j to n do V[j,r]:=v[j] od;
        fi;
        for j to r-1 do
          temp:=lincomb[j];
          for l from j+1 to r-1 do temp:=SIMPLIFY(temp+S[j,l]*lincomb[l]) od;
          S[j,r]:=-temp
        od;
        S[r,r]:=1;

        # compute A*v
        for i to n do
          temp:=0;
          for j to n do
            temp:=SIMPLIFY(temp+A[i,j]*v[j])
          od;
          u[i]:=temp
        od;
        v:=copy(u);
      else
        break
      fi
    od;

#######
# New cycle found
#######

    s:=array(1..r);
    for j to r do
      temp:=lincomb[j];
      for l from j+1 to r do temp:=SIMPLIFY(temp+S[j,l]*lincomb[l]) od;
      s[j]:=temp
    od;
    plist:=[op(plist),x^r-sum('s[r+1-j]*x^(r-j)','j'=1..r)]
#######
  od;

  if nargs=4 then
    Uinv:=inv(U,carrier);
    for i to n do
      for j to n do
        temp:=0;
        for l from i to n do temp:=SIMPLIFY(temp+S[i,l]*Uinv[l,j]) od;
        Vinv[i,j]:=temp
      od
    od
  fi;

  plist

end:


# A matrix B=plist_to_polycompanion(plist,x) is transformed to its Frobenius
# normal form F. If F=diag(C1,..,Cr), where Ci is the companion matrix
# associated with pi, then cyclic_to_frobenius will return the list
# [p1,..,pr].
# Let G be the matrix as described before. We compute the Smith normal
# form S of G. Then S=diag(p1,..,pr), where pi in K[x] such that pi
# divides p(i+1) for i=1..(r-1), and
# F=invfact_to_frobenius([p1,..,pr],x) is the Frobenius normal form
# of B (for a description of invfact_to_frobenius see below).
# Remark: to compute the Smith normal form of G we first simplify G using
# the fact that G is upper triangular. Then we use an adapted version of
# the Maple function smith.

`normform/cyclic_to_frobenius`:=proc(plist,x,T,Tinv)
local r,d,i,j,k,n,G,L,Linv,D,c,inv_fact,columnT,rowT,ii,jj,rr,q,
      columnTinv,rowTinv,US,S;

  r:=nops(plist);
  d:=array(0..r);
  d[0]:=0;
  for j to r do d[j]:=degree(plist[j],x) od;
  n:=d[r];

#######
# Compute matrix G
#######
  G:=zero_matrix(r,r);
  for j to r do
    for i to j-1 do
      G[i,j]:=sum('coeff(plist[j],x,k)*x^(k-d[i-1])','k'=d[i-1]..d[i]-1)
    od;
    G[j,j]:=sum('coeff(plist[j],x,k)*x^(k-d[j-1])','k'=d[j-1]..d[j])
  od;
#######

#######
# Compute Smith normal form of G
#######
  if nargs=2 then
    US:=uppersmith(G,x);
    S:=mysmith(US,x)
  elif nargs=3 then
    US:=uppersmith(G,x,'L');
    S:=mysmith(US,x,'L')
  else
    US:=uppersmith(G,x,'L','Linv');
    S:=mysmith(US,x,'L','Linv')
  fi;
#######

  D:=array(1..r);
  for i to r do D[i]:=degree(S[i,i],x) od;

  if nargs>=3 then
#######
# Compute transformation matrix (see diagram before)
#######
    c:=array(1..r);
    T:=array(1..n,1..n);
    columnT:=0;
    for i to r do
      for k to r do c[k]:=L[k,i] od;
      for j to D[i] do
        columnT:=columnT+1;
        for ii from r by -1 to 1 do
          q:=quo(c[ii],G[ii,ii],x,'rr');
          c[ii]:=SIMPLIFY(rr,x);
          for jj to ii-1 do
            c[jj]:=SIMPLIFY(c[jj]-q*G[jj,ii],x)
          od
        od;
        rowT:=0;
        for ii to r do
          for jj to d[ii]-d[ii-1] do
            rowT:=rowT+1;
            T[rowT,columnT]:=coeff(c[ii],x,jj-1)
          od
        od;
        for ii to r do c[ii]:=SIMPLIFY(c[ii]*x,x) od
      od
    od
#######
  fi;

  if nargs=4 then
#######
# Compute inverse transformation matrix (see diagram before)
#######
    Tinv:=array(1..n,1..n);
    columnTinv:=0;
    for i to r do
      for k to r do c[k]:=Linv[k,i] od;
      for j to d[i]-d[i-1] do
        columnTinv:=columnTinv+1;
        rowTinv:=0;
        for ii to r do
          c[ii]:=SIMPLIFY(rem(c[ii],S[ii,ii],x),x);
          for jj to D[ii] do
            rowTinv:=rowTinv+1;
            Tinv[rowTinv,columnTinv]:=coeff(c[ii],x,jj-1)
          od
        od;
        for ii to r do c[ii]:=SIMPLIFY(c[ii]*x,x) od
      od
    od
#######
  fi;

  inv_fact:=[];
  for i to r do
    if D[i]>0 then inv_fact:=[op(inv_fact),S[i,i]] fi
  od;

  inv_fact

end:


# An upper triangular matrix B is simplified. Entry B[i,j] is reduced
# modulo gcd(B[i,i],B[j,j]). If B' is the reduced matrix and L*B'*R=B
# then also L and L^(-1) are computed.

`normform/uppersmith`:=proc(B,x,L,Linv)
local i,j,k,n,r,s,t,A,d,q;

  A:=copy(B);
  n := linalg[rowdim](A);

  if nargs>=3 then
    L:=Id(n)
  fi;
  if nargs=4 then
    Linv:=Id(n)
  fi;

  for j from 2 to n do
    for i to j-1 do
      d:=GCDEX(A[i,i],A[j,j],x,'s','t');
      q:=quo(A[i,j],d,x,'r');
      A[i,j]:=SIMPLIFY(r,x);
      for k to i-1 do
        A[k,j]:=SIMPLIFY(A[k,j]-q*s*A[k,i],x)
      od;
      for k from j+1 to n do
        A[i,k]:=SIMPLIFY(A[i,k]-q*t*A[j,k],x)
      od;
      if nargs>=3 then
        for k to i do
          L[k,j]:=SIMPLIFY(L[k,j]+q*t*L[k,i],x)
        od
      fi;
      if nargs=4 then
        Linv[i,j]:=SIMPLIFY(-q*t,x)
      fi
    od
  od;

  op(A)

end:


# The Smith normal form S of a matrix B is computed. If L*S*R=B then
# also L and L^(-1) are computed. The matrix L computed in uppersmith is
# taken account of.
# For a description of mysmith see linalg[smith].
 
`normform/mysmith`:=proc(B,x,L,Linv)
local a,b,g,i,j,k,n,r,s,t,temp,A,isClear,q,lc;

  n:=linalg[rowdim](B);
  A:=copy(B);

  for k to n do
    isClear:=false;
    while not isClear do
      for i from k+1 to n do
        if A[i,k]=0 then next fi;
        g:=GCDEX(A[k,k],A[i,k],x,'s','t');
        a:=quo(A[k,k],g,x);b:=quo(A[i,k],g,x);
        for j from k+1 to n do
          temp:=SIMPLIFY(s*A[k,j]+t*A[i,j],x);
          A[i,j]:=SIMPLIFY(a*A[i,j]-b*A[k,j],x);
          A[k,j]:=temp
        od;
        if nargs>=3 then
          for j to n do
            temp:=SIMPLIFY(a*L[j,k]+b*L[j,i],x);
            L[j,i]:=SIMPLIFY(-t*L[j,k]+s*L[j,i],x);
            L[j,k]:=temp
          od
        fi;
        if nargs=4 then
          for j from k to n do
            temp:=SIMPLIFY(s*Linv[k,j]+t*Linv[i,j],x);
            Linv[i,j]:=SIMPLIFY(a*Linv[i,j]-b*Linv[k,j],x);
            Linv[k,j]:=temp
          od
        fi;
        A[k,k]:=SIMPLIFY(g,x);
        A[i,k]:=0
      od;
      isClear:=true;
      for i from k+1 to n do
        A[k,i]:=SIMPLIFY(rem(A[k,i],A[k,k],x,'q'),x);
      od;
      for i from k+1 to n do
        if A[k,i]=0 then next fi;
        g:=GCDEX(A[k,k],A[k,i],x,'s','t');
        a:=quo(A[k,k],g,x);b:=quo(A[k,i],g,x);
        for j from k+1 to n do
          temp:=SIMPLIFY(s*A[j,k]+t*A[j,i],x);
          A[j,i]:=SIMPLIFY(a*A[j,i]-b*A[j,k],x);
          A[j,k]:=temp
        od;
        A[k,k]:=SIMPLIFY(g,x);
        A[k,i]:=0;
        isClear:=false;
      od
    od
  od;
  r:=0;
  for i to n do
    if A[i,i]<>0 then
      r:=r+1;
      lc:=lcoeff(A[i,i],x);
      A[r,r]:=SIMPLIFY(A[i,i]/lc,x);
      if i<>r then
        A[i,i]:=0;
        if nargs>=3 then
          for j to n do
            temp:=L[j,r];
            L[j,r]:=L[j,i];
            L[j,i]:=temp
          od
        fi;
        if nargs=4 then
          for j to n do
            temp:=Linv[r,j];
            Linv[r,j]:=Linv[i,j];
            Linv[i,j]:=temp
          od
        fi
      fi
    fi
  od;
  for i to r-1 do
    for j from i+1 to r while A[i,i]<>1 do
      g:=GCDEX(A[i,i],A[j,j],x,'s','t');
      a:=quo(A[i,i],g,x); b:=quo(A[j,j],g,x);
      A[i,i]:=SIMPLIFY(g,x);
      A[j,j]:=SIMPLIFY( a*A[j,j],x );
      if nargs>=3 then
        for k to n do
          temp:=SIMPLIFY(a*L[k,i]+b*L[k,j],x);
          L[k,j]:=SIMPLIFY(-t*L[k,i]+s*L[k,j],x);
          L[k,i]:=temp
        od
      fi;
      if nargs=4 then
        for k to n do
          temp:=SIMPLIFY(s*Linv[i,k]+t*Linv[j,k],x);
          Linv[j,k]:=SIMPLIFY(a*Linv[j,k]-b*Linv[i,k],x);
          Linv[i,k]:=temp
        od
      fi
    od
  od;

  op(A)

end:


# inv computes the inverse of a permuted upper triangular matrix. The
# permutation is given by carrier.

`normform/inv`:=proc(A,carrier)
local B,n,i,j,k,temp;
  n:=linalg[rowdim](A);
  B:=array(1..n,1..n);
  for i to n do
    for j to i-1 do
      temp:=0;
      for k from j to i-1 do
        temp:=SIMPLIFY(temp+A[i,carrier[k]]*B[carrier[k],j])
      od;
      B[carrier[i],j]:=SIMPLIFY(-temp/A[i,carrier[i]])
    od;
    B[carrier[i],i]:=SIMPLIFY(1/A[i,carrier[i]]);
    for j from i+1 to n do
      B[carrier[i],j]:=0
    od
  od;
  op(B)
end:


# SIMPLIFY expands a polynomial with respect to x and normalizes its
# coefficients. According to the type of coefficients one of the following
# simpl* funcions is assigned to SIMPLIFY.

`normform/simplrational`:=proc(f,x)
  if nargs=1 then
    f
  else
    expand(f)
  fi
end:

`normform/simplcomplex`:=proc(f,x)
  if nargs=1 then
    evalc(f)
  else
    collect(f,x,evalc)
  fi
end:

`normform/simplalgebraic`:=proc(f,x)
  if nargs=1 then
    evala(normal(expand(f)))
  else
    collect(f,x,x->evala(normal(expand(x))))
  fi
end:

`normform/simplratfunc`:=proc(f,x)
  if nargs=1 then
    normal(f)
  else
    collect(f,x,normal)
  fi
end:

# gcdexgeneral is the extended euclidean algorithm. This routine is used
# in case the coefficients of the polynomials are not rational numbers.

`normform/gcdexgeneral`:=proc(f,g,x,s,t)
local c,d,c1,d1,c2,d2,q,r,r1,r2;
  c:=f;d:=g;
  c1:=1;d1:=0;
  c2:=0;d2:=1;
  while d<>0 do
    q:=quo(c,d,x,'r');
    r1:=c1-q*d1;r2:=c2-q*d2;
    c:=d;c1:=d1;c2:=d2;
    d:=SIMPLIFY(r);d1:=SIMPLIFY(r1);d2:=SIMPLIFY(r2)
  od;
  s:=c1/lcoeff(c,x);
  t:=c2/lcoeff(c,x);
  c/lcoeff(c,x)
end:


# zero_matrix creates a zero-matrix end Id creates an identity-matrix

`normform/zero_matrix`:=proc(r,c)
local A,i,j;
  A:=array(1..r,1..c);
  for i to r do
    for j to c do
      A[i,j]:=0
    od
  od;
  op(A)
end:

`normform/Id`:=proc(n)
local i,j,I;
  I:=array(1..n,1..n);
  for i to n do
    for j to n do
      I[i,j]:=0
    od
  od;
  for i to n do I[i,i]:=1 od;
  op(I)
end:


# basis creates an element of the natural basis of a vector space

`normform/basis`:=proc(n,i)
local b,j;
  b:=array(1..n);
  for j to n do b[j]:=0 od;
  b[i]:=1;
  op(b)
end:


# For plist=[p1,...,pr] where pi is a monic polynomial in x
# invfact_to_frobenius(plist,x) makes a square matrix with diagonal blocks
# C1,...,Cr where Ci is the companion matrix to pi.

`normform/invfact_to_frobenius`:=proc(inv_fact,x)
local i;
  linalg[diag](seq(linalg[companion](inv_fact[i],x),i=1..nops(inv_fact)))
end:


# If a=a0+a1*x+x^2, b=b0+b1*x+b2*x^2+x^3 and
# c=c0+c1*x+c2*x^2+c3*x^3+c4*x^4+x^5, then
# plist_to_polycompanion([a,b,c],x) yields
#
#       [ 0  -a0  -b0   0  -c0 ]
#       [                      ]
#       [ 1  -a1  -b1   0  -c1 ]
#       [                      ]
#       [ 0   0   -b2   0  -c2 ]
#       [                      ]
#       [ 0   0    0    0  -c3 ]
#       [                      ]
#       [ 0   0    0    1  -c4 ]

`normform/plist_to_polycompanion`:=proc(plist,x)
local r,d,n,A,i,j,k;
  r:=nops(plist);
  d:=array(0..r);
  d[0]:=0;
  for i to r do d[i]:=degree(plist[i],x) od;
  n:=d[r];
  A:=zero_matrix(n,n);
  for i to r do
    for j from d[i-1]+2 to d[i] do A[j,j-1]:=1 od;
    for j from i to r do
      for k from d[i-1]+1 to d[i] do
        A[k,d[j]]:=-coeff(plist[j],x,k-1)
      od
    od
  od;
  op(A)
end:


`help/text/frobenius` := TEXT(
`FUNCTION: frobenius - compute the Frobenius normal form of a matrix`,
`   `,
`CALLING SEQUENCE:`,
`   frobenius(A) or frobenius(A, K)`,
`   frobenius(A, 'P') or frobenius(A, K, 'P')`,
`   frobenius(A, 'P', 'Pinv') or frobenius(A, K, 'P', 'Pinv')`,
`   `,
`PARAMETERS:`,
`   A           - a square matrix`,
`   K           - an algebraic extension`,
`   'P', 'Pinv' - (optional) assigned the transformation matrix and its inverse`,
`   `,
`SYNOPSIS:`,
`- The function frobenius(A) computes and returns the Frobenius normal form`,
`  F of a matrix A.`,
`   `,
`- F has the following structure: F = diag(C1,C2,..,Ck) where the Ci's are com-`,
`  panion matrices associated with polynomials p1, p2,.., pk with the property`,
`  that pi divides p(i+1), for i = 1..k-1.`,
`   `,
`- If called in the form frobenius(A, 'P'), then P will be assigned the`,
`  transformation matrix corresponding to the Frobenius normal form, that is,`,
`  the matrix P such that inverse(P) * A * P = F.`,
`  If called in the form frobenius(A, 'P', 'Pinv'), then Pinv will be assigned`,
`  the inverse of P.`,
`   `,
`- If the optional parameter K is present, all calculations will be performed`,
`  in the algebraic number field defined by K. Here K is a set of RootOf's`,
`  and/or radicals`,
`   `,
`- When K is not present also rational functions in several variables are`,
`  allowed as matrix entries`,
`   `, 
`- The Frobenius normal form defined in this way is unique (ie. if we require`,
`  that pi divides p(i+1) as above).`,
`   `,
`EXAMPLES:`,
`> A := array([[-9,21,-15,4,2,0],[-10,21,-14,4,2,0],[-8,16,-11,4,2,0],`,
`>             [-6,12,-9,3,3,0],[-4,8,-6,0,5,0],[-2,4,-3,0,1,3]]);`,
`                              [  -9  21  -15  4  2  0 ]`,
`                              [                       ]`,
`                              [ -10  21  -14  4  2  0 ]`,
`                              [                       ]`,
`                              [  -8  16  -11  4  2  0 ]`,
`                         A := [                       ]`,
`                              [  -6  12   -9  3  3  0 ]`,
`                              [                       ]`,
`                              [  -4   8   -6  0  5  0 ]`,
`                              [                       ]`,
`                              [  -2   4   -3  0  1  3 ]`,
`   `,
`> frobenius(A,'P','Pinv');`,
`                             [ 3  0  0  0  0   0  ]`,
`                             [                    ]`,
`                             [ 0  0  0  0  0   15 ]`,
`                             [                    ]`,
`                             [ 0  1  0  0  0  -47 ]`,
`                             [                    ]`,
`                             [ 0  0  1  0  0   56 ]`,
`                             [                    ]`,
`                             [ 0  0  0  1  0  -32 ]`,
`                             [                    ]`,
`                             [ 0  0  0  0  1   9  ]`,
`   `,
`> op(P);op(Pinv);`,
`                    [ 3  23/8  29/8  -17/8  -227/8  -857/8 ]`,
`                    [                                      ]`,
`                    [ 3  19/8  21/8  -29/8  -235/8  -829/8 ]`,
`                    [                                      ]`,
`                    [ 3  15/8  17/8  -25/8  -199/8  -705/8 ]`,
`                    [                                      ]`,
`                    [ 3   3/2   3/2    -3     -21   -147/2 ]`,
`                    [                                      ]`,
`                    [ 3   7/8   5/8  -25/8  -139/8  -473/8 ]`,
`                    [                                      ]`,
`                    [ 2   1/2   1/2    -1     -7     -49/2 ]`,
`   `,
`                     [  0    0     0     -1/3    0    1  ]`,
`                     [                                   ]`,
`                     [  3  27/2  -33/2   -40/3   10   5  ]`,
`                     [                                   ]`,
`                     [ -7   -30    22    172/3  -33  -14 ]`,
`                     [                                   ]`,
`                     [  5   25    -13   -160/3   27   14 ]`,
`                     [                                   ]`,
`                     [ -1   -10    4      20     -9   -6 ]`,
`                     [                                   ]`,
`                     [  0   3/2   -1/2   -8/3    1    1  ]`,
`   `,
`> A := array([[3+I,1-6*I,2+3*I,I],`,
`              [5+2*I,5-I,4+2*I,3-I],`,
`              [2-I,2-I,3+2*I,5],`,
`              [6,7-2*I,3*I,8-4*I]]);`,
`                       [  3 + I   1 - 6 I  2 + 3 I     I    ]`,
`                       [                                    ]`,
`                       [ 5 + 2 I   5 - I   4 + 2 I   3 - I  ]`,
`                  A := [                                    ]`,
`                       [  2 - I    2 - I   3 + 2 I     5    ]`,
`                       [                                    ]`,
`                       [    6     7 - 2 I    3 I    8 - 4 I ]`,
`   `,
`> frobenius(A,{I});`,
`                           [ 0  0  0  299 - 1029 I ]`,
`                           [                       ]`,
`                           [ 1  0  0   181 + 267 I ]`,
`                           [                       ]`,
`                           [ 0  1  0   - 83 - 6 I  ]`,
`                           [                       ]`,
`                           [ 0  0  1    19 - 2 I   ]`,
`   `,
`> s:=sqrt(2):`,
`> A := array([[4*s-6,-4*s+7,-3*s+6],`,
`              [3*s-6,-3*s+7,-3*s+6],`,
`              [3*s,1-3*s,-2*s]]);`,
`                     [    1/2           1/2           1/2     ]`,
`                     [ 4 2    - 6  - 4 2    + 7  - 3 2    + 6 ]`,
`                     [                                        ]`,
`                     [    1/2           1/2           1/2     ]`,
`                A := [ 3 2    - 6  - 3 2    + 7  - 3 2    + 6 ]`,
`                     [                                        ]`,
`                     [      1/2            1/2          1/2   ]`,
`                     [   3 2        1 - 3 2        - 2 2      ]`,
`   `,
`> frobenius(A,{sqrt(2)});`,
`                           [  1/2                  ]`,
`                           [ 2     0        0      ]`,
`                           [                       ]`,
`                           [               1/2     ]`,
`                           [            4 2    - 7 ]`,
`                           [   0   0  2 ---------- ]`,
`                           [              1/2      ]`,
`                           [             2    - 2  ]`,
`                           [                       ]`,
`                           [              1/2      ]`,
`                           [           5 2    - 6  ]`,
`                           [   0   1   ----------  ]`,
`                           [             1/2       ]`,
`                           [            2    - 2   ]`,
`   `,
`> alias(a=RootOf(X^3-2*X+X-5)):`,
`> A := array([[11+6*a^2+2*a,6*a^2+10,-6*a^2-2*a-10],`,
`              [1+3*a+a^2,a+a^2,-3*a-a^2],`,
`              [4*a+6*a^2+10,6*a^2+10,-9-4*a-6*a^2]]);`,
`                  [         2           2            2            ]`,
`                  [ 11 + 6 a  + 2 a  6 a  + 10  - 6 a  - 2 a - 10 ]`,
`                  [                                               ]`,
`                  [              2          2                2    ]`,
`             A := [   1 + 3 a + a      a + a        - 3 a - a     ]`,
`                  [                                               ]`,
`                  [          2          2                       2 ]`,
`                  [ 4 a + 6 a  + 10  6 a  + 10   - 9 - 4 a - 6 a  ]`,
`   `,
`> frobenius(A,{a});`,
`                         [ 1 - 2 a  0        0       ]`,
`                         [                           ]`,
`                         [                     2     ]`,
`                         [    0     0  10 + 5 a  - a ]`,
`                         [                           ]`,
`                         [                        2  ]`,
`                         [    0     1    1 + a + a   ]`,
`   `,
`> A := array([[(y+y^2-x^2)/y,(x-x^2-y+y^2)/y,(x^2-y^2)/y],`,
`              [1+x+y,(x-y+y^2+x*y)/y,-x-y],`,
`              [(y-x+y^2-x^2)/y,(x-y+y^2-x^2)/y,(x+x^2-y^2)/y]]);`,
`                 [        2    2          2        2     2    2   ]`,
`                 [   y + y  - x      x - x  - y + y     x  - y    ]`,
`                 [   -----------     ---------------    -------   ]`,
`                 [        y                 y              y      ]`,
`                 [                                                ]`,
`                 [                           2                    ]`,
`                 [                  x - y + y  + x y              ]`,
`            A := [    1 + x + y     ----------------    - x - y   ]`,
`                 [                          y                     ]`,
`                 [                                                ]`,
`                 [          2    2        2        2       2    2 ]`,
`                 [ y - x + y  - x    x - x  - y + y   x + x  - y  ]`,
`                 [ ---------------   ---------------  ----------- ]`,
`                 [        y                 y              y      ]`,
`   `,
`> frobenius(A);`,
`                            [ x/y  0        0      ]`,
`                            [                      ]`,
`                            [            x (x + y) ]`,
`                            [  0   0   - --------- ]`,
`                            [                y     ]`,
`                            [                      ]`,
`                            [                    2 ]`,
`                            [         x + x y + y  ]`,
`                            [  0   1  ------------ ]`,
`                            [               y      ]`,
`   `,
`SEE ALSO:  smithex, ismithex, ratjordan, jordansymbolic, jordan,`,
`           Frobenius, Ratjordan, Jordansymbolic`  
):



############################################################################
############################################################################
##
##          ratjordan
##
###########################################################################
###########################################################################
# A Maple program for the computation of the rational Jordan normal form
# of a matrix.
# Authors: T.M.L. Mulders, A.H.M. Levelt
#          Mathematics Department
#          University of Nijmegen.
# E-mail: mulders@sci.kun.nl, ahml@sci.kun.nl
#
# January 1993


# A primary invariant is a (non-empty) list
# prim_inv:=[[q1,[e11,e12,...]],[q2,[e21,e22,...]],....]
# where q1,q2,... are monic, irreducible, different polynomials in K[x],
# (K a field), and for each i [ei1,ei2,...] a non-empty list of positive
# integers.
# Conventions adopted: i->degree(qi) is non-decreasing and
# for each i, j->eij is non-decreasing.
#
# The matrix R in rational Jordan normal form corresponding to prim_inv
# is the square matrix with blocks
# ratj(q1,e11),ratj(q1,e12),...,ratj(q2,e21),ratj(q2,e22),...
# along the diagonal and zeroes elsewhere.
# Here
#                [C(p)  I             ]
#                [    C(p)  I         ]
#   ratj(p,e) =  [          .   .     ]
#                [            C(p)  I ]
#                [                C(p)]
# with e blocks C(p) along the diagonal. C(p) is the companion matrix
# corresponding to the monic polynomial p in K[x].
# If A is a square matrix over a field K, then there exist square matrices
# P and R over K such that R is in rational Jordan normal form and
#               inverse(P)*A*P = R.
# The matrix R is called the rational Jordan normal form of A.
#
# The function ratjordan computes the rational Jordan normal form R of
# a matrix A, the transformation matrix P and its inverse P^(-1).
# Specifically:
# - ratjordan(A) or ratjordan(A,K) will return the rational Jordan normal
#   form R of A.
# - ratjordan(A,'P') or ratjordan(A,K,'P') will do the same as ratjordan(A)
#   (resp. ratjordan(A,K)), but now the transformation matrix is assigned to P.
# - ratjordan(A,'P','Pinv') or ratjordan(A,K,'P','Pinv') will do the same
#   as ratjordan(A,'P') (resp. ratjordan(A,K,'P')), but now also the inverse
#   of the transformation matrix is assigned to Pinv.
# Here K is a set of RootOf's and/or radicals defining an algebraic extension
# of Q(the rational numbers).
#
# Global description of the algorithm:
# For a given n by n matrix A over a field K, we first compute the
# Frobenius normal form F of A. Then we compute the rational Jordan
# normal form of F, which is also the rational Jordan normal form of A.
# If F=diag(C1,..,Cr), where Ci is the companion matrix associated with a
# polynomial pi in K[x], we first compute the rational Jordan normal form
# of C1 to Cr. From these we then extract the rational Jordan normal form
# of F.


ratjordan:=proc(A)
local AA,n,i,j;

  if not type(A,'matrix') then
    AA:=evalm(A)
  else
    AA:=A
  fi;
  if not type(AA,'matrix'('anything','square')) then
    ERROR(`expecting a square matrix`)
  fi;

  n:=linalg[rowdim](AA);
  for i to n do
    for j to n do
      if type(AA[i,j],indexed) then
        ERROR(`Unassigned array elements`)
      fi
    od
  od;

  if nargs>1 and type(args[2],set) then
    if args[2]={I} then
      SIMPLIFY:=simplcomplex;
      GCDEX:=gcdexgeneral;
      MULTIPLE:=multiplegeneral;
      ratjordanform(AA,args[2..nargs])
    else
      SIMPLIFY:=simplalgebraic;
      GCDEX:=gcdexgeneral;
      MULTIPLE:=multiplegeneral;
      ratjordanform(AA,args[2..nargs])
    fi
  else
    if type(AA,'matrix'('rational')) then
      SIMPLIFY:=simplrational;
      GCDEX:=gcdex;
      MULTIPLE:=lcm;
      ratjordanform(AA,{},args[2..nargs])
    else
      SIMPLIFY:=simplratfunc;
      GCDEX:=gcdexgeneral;
      MULTIPLE:=multiplegeneral;
      ratjordanform(AA,{},args[2..nargs])
    fi
  fi

end:

`normform/ratjordanform`:=proc(A,K,P,Pinv)
local F,prim_inv,x,T,Tinv,S,Sinv;

  if nargs=2 then
    F:=frobeniusform(A);
    prim_inv:=frobenius_to_ratjordan(F,K,x)
  elif nargs=3 then
    F:=frobeniusform(A,'T');
    prim_inv:=frobenius_to_ratjordan(F,K,x,'S');
    P:=map(SIMPLIFY,evalm(T&*S))
  else
    F:=frobeniusform(A,'T','Tinv');
    prim_inv:=frobenius_to_ratjordan(F,K,x,'S','Sinv');
    P:=map(SIMPLIFY,evalm(T&*S));
    Pinv:=map(SIMPLIFY,evalm(Sinv&*Tinv))
  fi;

  priminv_to_ratjordan(prim_inv,x)

end:


# frobenius_to_ratjordan computes the rational Jordan normal form R of a
# matrix F which is in Frobenius normal form. Say F=diag(C1,..,Cr), where
# Ci is the companion matrix associated with the polynomial pi. First we
# determine the irreducible factors P1,..,PN which appear in p1 through
# pr and build a matrix fact_mat such that pi=
# product(Pj^fact_mat[i,j],j=1..N). This matrix is used at several places
# in the algorithm.
# In fact we can immediately extract from fact_mat the rational Jordan
# normal form of F. If also the transformation matrix is wanted, we compute
# it first for C1 to Cr. Then we compute the transformation matrix by
# rearranging the former results.
# If R is the matrix in rational Jordan normal form corresponding to
# prim_inv:=[[q1,[e11,e12,...]],[q2,[e21,e22,...]],....], then
# prim_inv is returned by frobenius_to_ratjordan.


`normform/frobenius_to_ratjordan`:=proc(F,K,x,S,Sinv)
local P,inv_fact,g,L,h,fact_mat,r,N,T_list,i,j,k,facts,T,n,cols,prim_inv,
      exp_list,G,p,e,Tinv_list,Q,Qinv,d,degp,count,Tinv,m;

  # compute p1,..,pr
  inv_fact:=frobenius_to_invfact(F,x);
  r:=nops(inv_fact);

#######
# Compute fact_mat
#######
  g:=[inv_fact[1],seq(SIMPLIFY(quo(inv_fact[i],inv_fact[i-1],x),x),i=2..r)];
  L:=[];
  for i to r do
    m:=MULTIPLE(seq(denom(coeff(g[i],x,j)),j=0..degree(g[i],x)));
    h:=factors(SIMPLIFY(m*g[i],x),K)[2];
    L:=[op(L),seq([i,SIMPLIFY(h[j][1]/lcoeff(h[j][1],x),x),h[j][2]],j=1..nops(h))]
  od;
  P:=deg_sort([op({seq(L[i][2],i=1..nops(L))})],x);
  N:=nops(P);
  G:=array(1..r,1..N);
  fact_mat:=array(1..r,1..N);
  for i to r do for j to N do G[i,j]:=0; fact_mat[i,j]:=0 od od;
  for k to nops(L) do
    i:=L[k][1];
    p:=L[k][2];
    e:=L[k][3];
    for j to N do
      if p=P[j] then break fi
    od;
    G[i,j]:=e
  od;
  for j to N do fact_mat[1,j]:=G[1,j] od;
  for i from 2 to r do
    for j to N do
      fact_mat[i,j]:=fact_mat[i-1,j]+G[i,j]
    od
  od;
#######

  if nargs>=4 then
#######
# Compute transition matrix for C1 through Cr
#######
    T_list:=[];
    if nargs=5 then
      Tinv_list:=[]
    fi;
    for i to r do
      facts:=[];
      for j to N do
        if fact_mat[i,j]<>0 then facts:=[op(facts),[P[j],fact_mat[i,j]]] fi
      od;
      if nargs=4 then
        companion_to_ratjordan(facts,x,inv_fact[i],'Q')
      else
        companion_to_ratjordan(facts,x,inv_fact[i],'Q','Qinv');
        Tinv_list:=[op(Tinv_list),op(Qinv)]
      fi;
      T_list:=[op(T_list),op(Q)];
    od;
#######

#######
# Compute transition matrix by permuting diag(T_list[1],..,T_list[r])
#######
    d:=array(1..r,1..N);
    degp:=array(1..r);
    for i to r do
      for j to N do
        d[i,j]:=degree(P[j],x)*fact_mat[i,j]
      od;
      degp[i]:=sum('d[i,j]','j'=1..N)
    od;
    cols:=[];
    for j to N do
      for i to r do
        count:=sum('degp[k]','k'=1..i-1)+sum('d[i,k]','k'=1..j-1);
        for h to d[i,j] do
          cols:=[op(cols),count+h]
        od
      od
    od;

    T:=linalg[diag](op(T_list));
    n:=linalg[rowdim](T);
    S:=array(1..n,1..n);
    for i to n do
      for j to n do
        S[i,j]:=T[i,cols[j]]
      od
    od;

    if nargs=5 then
      Tinv:=linalg[diag](op(Tinv_list));
      Sinv:=array(1..n,1..n);
      for i to n do
        for j to n do
          Sinv[i,j]:=Tinv[cols[i],j]
        od
      od
    fi
#######
  fi;

#######
# Compute prim_inv
#######
  prim_inv:=[];
  for j to N do
    exp_list:=[];
    for i to r do
      if fact_mat[i,j]<>0 then exp_list:=[op(exp_list),fact_mat[i,j]] fi
    od;
    prim_inv:=[op(prim_inv),[P[j],exp_list]]
  od;
#######

  prim_inv

end:

`normform/deg_sort`:=proc(l,x)
local ll,n,i,j;
  ll:=l;
  n:=nops(ll);
  for i from 1 to nops(ll)-1 do
    for j from i+1 to nops(ll) do
      if degree(ll[j],x)<degree(ll[i],x) then
        ll:=[op(1..i-1,ll),ll[j],op(i..j-1,ll),op(j+1..n,ll)]
      fi
    od
  od;
  ll
end:


# companion_to_ratjordan computes the rational Jordan normal form of a
# matrix C which is the companion matrix of a polynomial p. Since the
# factors of p are known, the rational Jordan normal form of C is also
# known, so in fact we only have to compute the transition matrix.
#
# Global description of the algorithm:
# First consider the case where p=q^e, q irreducible. Let n=degree(p). Then
# we have the following diagram:
#                           ~
#                   K^n <------- K[x]/q^e
#
#                    |               |
#                    |               |
#                    |C              |x
#                    |               |
#                    |               |
#                   \ /             \ /
#                           ~
#                   K^n <------- K[x]/q^e
#
# We look for a K-basis (b1,..,bn) of K[x]/q^e such that we get the
# following diagram:
#                       ~                ~
#               K^n <------- K[x]/q^e -------> K^n
#
#                |               |              |
#                |               |              |
#                |C              |x             |ratj(q,e)
#                |               |              |
#                |               |              |
#               \ /             \ /            \ /
#                       ~                ~
#               K^n <------- K[x]/q^e -------> K^n
#
# Let q=x^d+q(d-1)*x^(d-1)+..+q1*x+q0. It follows that b1,..,bn must satisfy
# the following relations:
#
# x*b1      = b2
# x*b2      = b3
# ...
# x*bd      = -q0*b1-q1*b2-..-q(d-1)*bd
# x*b(d+1)  = b(d+2)+b1
# x*b(d+2)  = b(d+3)+b2
# ...
# x*b(2d)   = -q0*b(d+1)-q1*b(d+2)-..-q(d-1)*b(2d)+bd
# x*b(2d+1) = b(2d+2)+b(d+1)
# ...
# x*bn      = -q0*b(n-d+1)-q1*b(n-d+2)-..-q(d-1)*bn+b(n-d)
# From this we deduce that b1,b(d+1),b(2d+1),... must satisfy the following
# relations:
#
# q*b1      = 0
# q*b(d+1)  = q'*b1
# q*b(2d+1) = q'*b(d+1)-1/2*q''*b1
# q*b(3d+1) = q'*b(2d+1)-1/2*q''*b(d+1)+1/6*q'''*b1
# q*b(4d+1) = q'*b(3d+1)-1/2*q''*b(2d+1)+1/6*q'''*b(d+1)-1/24*q''''*b1
# ...
# where ' stands for taking the derivative with respect to x.
# If we choose b1=q^(e-1) we can compute b2,..,bn from the relations above.
# We assume that K is a perfect field, so q' is not zero. From this we
# see that q^(e-i-1) divides b(id+1) while q^(e-i) does not divide
# b(di+1). In particular we have gcd(b((e-1)i+1),q)=1.
# Notice also the following relations which can be easily proved:
# x^i*b1      = b(i+1)
# x^i*b(d+1)  = b(d+i+1)+binomial(i,1)*bi
# x^i*b(2d+1) = b(2d+i+1)+binomial(i,1)*b(d+i)+binomial(i,2)*b(i-1)
# ... 
#
# Now the general case where p=q1^e1*q2^e2*..*qr^er. To compose the partial
# results we use the following diagram:
#       ~          ~                               ~
# K^n <--- K[x]/p ---> K[x]/q1^e1 X..X K[x]/qr^er ---> K^n1 X......X K^nr
#
#  |          |            |               |            |             |
#  |          |            |               |            |             |
#  |C         |x           |x              |x           |ratj(q1,e1)  |ratj(qr,er)
#  |          |            |               |            |             |
#  |          |            |               |            |             |
# \ /        \ /          \ /             \ /          \ /           \ /
#       ~          ~                               ~
# K^n <--- K[x]/p ---> K[x]/q1^e1 X..X K[x]/qr^er ---> K^n1 X......X K^nr
#
# In order to compose the K_bases of K[x]/q1^e1 through K[x]/qr^er to a
# K-basis of K[x]/p we compute polynomials u1,..,ur such that
# (ui mod qi^ei)=1 and (ui mod qj^ej)=0.

`normform/companion_to_ratjordan`:=proc(fact_list,x,f,Q,Qinv)
local i,j,k,r,g_list,u_list,bbasis,q,e,d,qpower,diffq,
      part_basis,ratj_basis,n,s,t,g,rowQinv,pol_lincomb,qq,rr,
      lincomb,index,v,u,a;

  r:=nops(fact_list);
  n:=degree(f,x);

  g_list:=[seq(SIMPLIFY(fact_list[i][1]^fact_list[i][2],x),i=1..r)];

#######
# Compute u1,..,ur
#######
  u_list:=array(1..r);
  if r=1 then u_list[1]:=1
  else
    GCDEX(g_list[1],g_list[2],x,'s','t');
    u_list[1]:=SIMPLIFY(t*g_list[2],x);
    u_list[2]:=SIMPLIFY(s*g_list[1],x);
    g:=SIMPLIFY(g_list[1]*g_list[2],x);
    for i from 3 to r do
      GCDEX(g,g_list[i],x,'s','t');
      for j to i-1 do
        u_list[j]:=SIMPLIFY(rem(u_list[j]*t*g_list[i],f,x),x)
      od;
      u_list[i]:=SIMPLIFY(s*g,x);
      g:=SIMPLIFY(g*g_list[i],x)
    od
  fi;
#######

  bbasis:=[];  # basis will contain a K-basis of K[x]/f
  rowQinv:=0;

  Q:=array(1..n,1..n);
  if nargs=5 then
    Qinv:=array(1..n,1..n)
  fi;

  for i to r do
    q:=fact_list[i][1];
    e:=fact_list[i][2];
    d:=degree(q,x);

    qpower:=array(1..e+1);
    qpower[1]:=1;
    for j from 2 to e+1 do qpower[j]:=SIMPLIFY(q*qpower[j-1],x) od;

    if e>1 then
      diffq:=array(1..e-1);
      diffq[1]:=SIMPLIFY(diff(q,x),x);
      for j from 2 to e-1 do diffq[j]:=SIMPLIFY(diff(diffq[j-1],x),x) od
    fi;

#######
# Compute b1,b(d+1),b(2d+1),...
#######
    part_basis:=array(1..e);
    part_basis[1]:=SIMPLIFY(q^(e-1),x);
    for j from 2 to e do
      part_basis[j]:=SIMPLIFY(normal(sum('(-1)^(k-1)/(k!)*diffq[k]*part_basis[j-k]','k'=1..j-1)/q),x)
    od;
#######

#######
# Compute b1,..,bni
#######
    ratj_basis:=array(1..e*d);
    ratj_basis[1]:=part_basis[1];
    for k from 2 to d do
      ratj_basis[k]:=SIMPLIFY(x*ratj_basis[k-1],x)
    od;
    for j from 2 to e do
      ratj_basis[(j-1)*d+1]:=part_basis[j];
      for k from 2 to d do
        ratj_basis[(j-1)*d+k]:=SIMPLIFY(x*ratj_basis[(j-1)*d+k-1]-ratj_basis[(j-2)*d+k-1],x)
      od;
    od;
#######

#######
# Complete basis
#######
    for k to e*d do
      t:=SIMPLIFY(rem(u_list[i]*ratj_basis[k],f,x),x);
      bbasis:=[op(bbasis),t]
    od;
#######

    if nargs=5 then
#######
# Compute next e*d rows of Qinv (see diagram above)
#######

  #######
  # Compute coordinates of 1 with respect to basis (b1,..,bn)
  # Use the fact that q^(e-i-1) divides b(id+1) and gcd(b((e-1)d+1),q)=1
  #######
      pol_lincomb:=array(1..e);
      for j to e do pol_lincomb[j]:=0 od;
      GCDEX(part_basis[e],qpower[e+1],x,'s','t');  # =1
      pol_lincomb[e]:=SIMPLIFY(s,x);
      for j from e by -1 to 1 do
        qq:=quo(pol_lincomb[j],q,x,'rr');
        pol_lincomb[j]:=SIMPLIFY(rr,x);
        for k to j-1 do
          pol_lincomb[j-k]:=SIMPLIFY(rem(pol_lincomb[j-k]+qq*diffq[k]*(-1)^(k-1)/k!,qpower[j+1],x),x)
        od
      od;
      lincomb:=array(1..e*d);
      for j to e do
        for k to d do
          index:=(j-1)*d+k;
          lincomb[index]:=coeff(pol_lincomb[j],x,k-1);
          for v to min(j-1,k-1) do
            lincomb[index-v*d-v]:=SIMPLIFY(lincomb[index-v*d-v]+coeff(pol_lincomb[j],x,k-1)*binomial(k-1,v))
          od
        od
      od;

      for u to e*d do
        rowQinv:=rowQinv+1;
        Qinv[rowQinv,1]:=lincomb[u]
      od;
  #######

  #######
  # Compute coordinates of x^v with respect to basis (b1,..,bn)
  #######
      for v from 2 to n do
        a:=copy(lincomb);
        index:=0;
        for j to e-1 do
          index:=index+1;
          lincomb[index]:=SIMPLIFY(-coeff(q,x,0)*a[j*d]+a[j*d+1]);
          for k from 2 to d do
            index:=index+1;
            lincomb[index]:=SIMPLIFY(a[(j-1)*d+k-1]-coeff(q,x,k-1)*a[j*d]+a[j*d+k])
          od
        od;
        index:=index+1;
        lincomb[index]:=SIMPLIFY(-coeff(q,x,0)*a[e*d]);
        for k from 2 to d do
          index:=index+1;
          lincomb[index]:=SIMPLIFY(a[(e-1)*d+k-1]-coeff(q,x,k-1)*a[e*d])
        od;

        rowQinv:=rowQinv-e*d;
        for u to e*d do
          rowQinv:=rowQinv+1;
          Qinv[rowQinv,v]:=lincomb[u]
        od

      od
  #######

#######
    fi
  od;

#######
# Compute Q (see diagram above)
#######
  for j to n do
    for k to n do
    Q[k,j]:=coeff(bbasis[j],x,k-1)
    od
  od;
#######

  NULL
end:


# For a matrix F in Frobenius normal form, frobenius_to_invfact(F,x) computes
# the list inv_fact:=[p1,..,pr] such that F=invfact_to_frobenius(plist,x)

`normform/frobenius_to_invfact`:=proc(F,x)
local n,k,p,i,j,inv_fact;
  n:=linalg[rowdim](F);
  inv_fact:=[];
  k:=1;
  while k<=n do
    p:=0;
    i:=k+1;
    while i<=n and F[i,i-1]=1 do i:=i+1 od;
    for j from k to i-1 do
      p:=p-F[j,i-1]*x^(j-k)
    od;
    p:=sort(p+x^(i-k));
    inv_fact:=[op(inv_fact),p];
    k:=i
  od;
  inv_fact
end:


# For a primary invariant prim_inv, priminv_to_ratjordan(prim_inv,x) returns
# the matrix R in rational Jordan normal form corresponding to prim_inv

`normform/priminv_to_ratjordan`:=proc(prim_inv,x)
local r,i,j,p,exp_list,block_list;
  r:=nops(prim_inv);
  block_list:=[];
  for i to r do
    p:=prim_inv[i][1];
    exp_list:=prim_inv[i][2];
    for j to nops(exp_list) do
      block_list:=[op(block_list), make_ratj_block(p,x,exp_list[j])]
    od
  od;
  linalg[diag](op(block_list))
end:

# For a monic polynomial p in x and a positive integer e,
# make_ratj_block(p,x,e) returns the matrix ratj(p,e)

`normform/make_ratj_block`:=proc(p,x,e)
local C,d,n,J_block,i;
  C:=linalg[companion](p,x);
  d:=degree(p,x);
  n:=d*e;
  J_block:=zero_matrix(n,n);
  for i to e do
    linalg[copyinto](C,J_block,(i-1)*d+1,(i-1)*d+1)
  od;
  for i to n-d do
    J_block[i,i+d]:=1
  od;
  op(J_block)
end:


# multiplegeneral computes the product of the arguments

`normform/multiplegeneral`:=proc()
local i;
  SIMPLIFY(product('args[i]','i'=1..nargs))
end:

`help/text/ratjordan` := TEXT(
`FUNCTION: ratjordan - compute the rational Jordan normal form of a matrix`,
`   `,
`CALLING SEQUENCE:`,
`   ratjordan(A) or ratjordan(A, K)`,
`   ratjordan(A, 'P') or ratjordan(A, K, 'P')`,
`   ratjordan(A, 'P', 'Pinv') or ratjordan(A, K, 'P', 'Pinv')`,
`   `,
`PARAMETERS:`,
`   A          - a square matrix`,
`   K          - an algebraic extension`,
`   'P','Pinv' - (optional) assigned the transformation matrix and its inverse`,
`   `,
`SYNOPSIS:`,
`- The function ratjordan(A) computes and returns the rational Jordan normal`,
`  form R of a matrix A.`,
`   `,
`- R has the following structure: R = diag(R11,R12,..,R21,R22,..) where the`,
`  Rij's have the following shape:`,
`   `,
`             [ C(pi)   I                     ]`,
`             [                               ]`,
`             [       C(pi)   I               ]`,
`             [                               ]`,
`             [               .     .         ]`,
`             [                               ]`,
`             [                   C(pi)   I   ]`,
`             [                               ]`,
`             [                         C(pi) ]`,
`   `,
`  where there are eij blocks C(pi) along the diagonal and C(pi) is the`,
`  companion matrix associated with the irreducible polynomial pi.`,
`  Convention: i->degree(pi) is non-decreasing and for each i, j->eij is`,
`  non_decreasing`,
`  `,
`- If called in the form ratjordan(A, 'P'), then P will be assigned the`,
`  transformation matrix corresponding to the rational Jordan normal form,`,
`  that is, the matrix P such that inverse(P) * A * P = R.`,
`  If called in the form ratjordan(A, 'P', 'Pinv'), then Pinv will be assigned`,
`  the inverse of P.`,
`   `,
`- If the optional parameter K is present, all calculations will be performed`,
`  in the algebraic number field defined by K. Here K is a set of RootOf's`,
`  and/or radicals`,
`   `,
`- When K is not present also rational functions in several variables are`,
`  allowed as matrix entries`,
`   `,
`EXAMPLES:`,
`> A := array([[-9,21,-15,4,2,0],[-10,21,-14,4,2,0],[-8,16,-11,4,2,0],`,
`>             [-6,12,-9,3,3,0],[-4,8,-6,0,5,0],[-2,4,-3,0,1,3]]);`,
`                              [  -9  21  -15  4  2  0 ]`,
`                              [                       ]`,
`                              [ -10  21  -14  4  2  0 ]`,
`                              [                       ]`,
`                              [  -8  16  -11  4  2  0 ]`,
`                         A := [                       ]`,
`                              [  -6  12   -9  3  3  0 ]`,
`                              [                       ]`,
`                              [  -4   8   -6  0  5  0 ]`,
`                              [                       ]`,
`                              [  -2   4   -3  0  1  3 ]`,
`   `,
`> ratjordan(A,'P','Pinv');`,
`                             [ 1  1  0  0  0   0 ]`,
`                             [                   ]`,
`                             [ 0  1  0  0  0   0 ]`,
`                             [                   ]`,
`                             [ 0  0  3  0  0   0 ]`,
`                             [                   ]`,
`                             [ 0  0  0  3  0   0 ]`,
`                             [                   ]`,
`                             [ 0  0  0  0  0  -5 ]`,
`                             [                   ]`,
`                             [ 0  0  0  0  1   4 ]`,
`   `,
`> op(P);op(Pinv);`,
`                        [  1   1/4  3  -3/8   3   7/2 ]`,
`                        [                             ]`,
`                        [  1   1/4  3  -3/8  5/2  5/2 ]`,
`                        [                             ]`,
`                        [  1   1/4  3  -3/8   2    2  ]`,
`                        [                             ]`,
`                        [ 3/4  3/8  3  -3/8  3/2  3/2 ]`,
`                        [                             ]`,
`                        [ 1/2  1/4  3  -3/8   1    1  ]`,
`                        [                             ]`,
`                        [ 1/4  1/8  2  -1/8  1/2  1/2 ]`,
`   `,
`                          [  0  -4   6    0   -2  0 ]`,
`                          [                         ]`,
`                          [  0   0  -4    8   -4  0 ]`,
`                          [                         ]`,
`                          [  0   0   0  -1/3   0  1 ]`,
`                          [                         ]`,
`                          [  0   0   0   8/3  -8  8 ]`,
`                          [                         ]`,
`                          [ -2   6  -4    0    0  0 ]`,
`                          [                         ]`,
`                          [  2  -4   2    0    0  0 ]`,
`   `,
`> A := array([[-3-I,1,2+I,7-9*I],`,
`              [-2,1,1,5-I],`,
`              [-2-2*I,1,2+2*I,4-2*I],`,
`              [2,0,-1,-2+8*I]]);`,
`                        [  - 3 - I   1   2 + I    7 - 9 I  ]`,
`                        [                                  ]`,
`                        [     -2     1     1       5 - I   ]`,
`                   A := [                                  ]`,
`                        [ - 2 - 2 I  1  2 + 2 I   4 - 2 I  ]`,
`                        [                                  ]`,
`                        [     2      0     -1    - 2 + 8 I ]`,
`   `,
`> ratjordan(A,{I});`,
`                         [ 1 + I    0    0      0     ]`,
`                         [                            ]`,
`                         [   0    1 + I  0      0     ]`,
`                         [                            ]`,
`                         [   0      0    0  - 2 - 5 I ]`,
`                         [                            ]`,
`                         [   0      0    1  - 4 + 7 I ]`,
`   `,
`> s:=sqrt(2):`,
`> A := array([[4*s-6,-4*s+7,-3*s+6],`,
`              [3*s-6,-3*s+7,-3*s+6],`,
`              [3*s,1-3*s,-2*s]]);`,
`                     [    1/2           1/2           1/2     ]`,
`                     [ 4 2    - 6  - 4 2    + 7  - 3 2    + 6 ]`,
`                     [                                        ]`,
`                     [    1/2           1/2           1/2     ]`,
`                A := [ 3 2    - 6  - 3 2    + 7  - 3 2    + 6 ]`,
`                     [                                        ]`,
`                     [      1/2            1/2          1/2   ]`,
`                     [   3 2        1 - 3 2        - 2 2      ]`,
`   `,
`> ratjordan(A,{sqrt(2)});`,
`                           [        1/2             ]`,
`                           [ 1 - 3 2       0     0  ]`,
`                           [                        ]`,
`                           [              1/2       ]`,
`                           [      0      2       0  ]`,
`                           [                        ]`,
`                           [                    1/2 ]`,
`                           [      0        0   2    ]`,
`   `,
`> alias(a=RootOf(X^3-2*X+X-5)):`,
`> A := array([[11+6*a^2+2*a,6*a^2+10,-6*a^2-2*a-10],`,
`              [1+3*a+a^2,a+a^2,-3*a-a^2],`,
`              [4*a+6*a^2+10,6*a^2+10,-9-4*a-6*a^2]]);`,
`                  [         2           2            2            ]`,
`                  [ 11 + 6 a  + 2 a  6 a  + 10  - 6 a  - 2 a - 10 ]`,
`                  [                                               ]`,
`                  [              2          2                2    ]`,
`             A := [   1 + 3 a + a      a + a        - 3 a - a     ]`,
`                  [                                               ]`,
`                  [          2          2                       2 ]`,
`                  [ 4 a + 6 a  + 10  6 a  + 10   - 9 - 4 a - 6 a  ]`,
`   `,
`> ratjordan(A,{a});`,
`                         [ 1 - 2 a     0         0    ]`,
`                         [                            ]`,
`                         [    0     1 - 2 a      0    ]`,
`                         [                            ]`,
`                         [                          2 ]`,
`                         [    0        0     3 a + a  ]`,
`   `,
`> A := array([[(y+y^2-x^2)/y,(x-x^2-y+y^2)/y,(x^2-y^2)/y],`,
`              [1+x+y,(x-y+y^2+x*y)/y,-x-y],`,
`              [(y-x+y^2-x^2)/y,(x-y+y^2-x^2)/y,(x+x^2-y^2)/y]]);`,
`               [         2    2             2        2     2    2   ]`,
`               [    y - x  + y       - y - x  + x + y     x  - y    ]`,
`               [    -----------      -----------------    -------   ]`,
`               [         y                   y               y      ]`,
`               [                                                    ]`,
`               [                               2                    ]`,
`               [                    - y + x + y  + x y              ]`,
`          A := [     1 + y + x      ------------------    - y - x   ]`,
`               [                             y                      ]`,
`               [                                                    ]`,
`               [            2    2          2        2       2    2 ]`,
`               [ - x + y - x  + y    - y - x  + x + y   x + x  - y  ]`,
`               [ -----------------   -----------------  ----------- ]`,
`               [         y                   y               y      ]`,
`   `,
`> ratjordan(A);`,
`                              [ x + y   0    0  ]`,
`                              [                 ]`,
`                              [   0    x/y   0  ]`,
`                              [                 ]`,
`                              [   0     0   x/y ]`,
`   `,
`SEE ALSO: smithex, ismithex, frobenius, jordansymbolic, jordan,`,
`          Frobenius, Ratjordan, Jordansymbolic`
):



############################################################################
############################################################################
##
##          jordansymbolic and jordan
##
###########################################################################
###########################################################################
# A Maple program for the computation of the Jordan normal form of a matrix.
# Authors: T.M.L. Mulders, A.H.M. Levelt
#          Mathematics Department
#          University of Nijmegen.
# E-mail: mulders@sci.kun.nl, ahml@sci.kun.nl
#
# January 1993


# An invariant is a (non_empty) list
# invariant:=[[x1,[e11,e12,...]],[x2,[e21,e22,...]],....]
# where xi in K (K a field), and for each i [ei1,ei2,...] a non-empty
# list of positive integers.
# Convention adopted: for each i, j->eij is non_decreasing.
#
# The matrix J in Jordan normal form corresponding to invariant is the
# square matrix with blocks
# jord(x1,e11),jord(x1,e12),...,jord(x2,e21),jord(x2,e22),...
# along the diagonal and zeroes elsewhere.
# Here
#              [x 1      ]
#              [  x 1    ]
#  jord(x,e) = [    . .  ]
#              [      x 1]
#              [        x]
# with e times x along the diagonal.
# If A is a square matrix over a field K, and the characteristic polynomial
# of A splits completely over K, then there exist square matrices
# P and J over K such that J is in Jordan normal form and
#               inverse(P)*A*P = J.
# The matrix J is called the Jordan normal form of A.
# If the characteristic polynomial p of A does not split completely in K
# we can still compute the Jordan normal form of A as it would be in
# a splitting field L of p over K. We will give the zeroes of p in L\K
# symbolic names. These names will then appear in both J and P. If K=Q
# (the rational numbers) or some algebraic extension of Q we will also
#  compute the Jordan normal form of A in C (the complex numbers). The zeroes
# of p will be computed exactly if possible. Zeroes which are not computed
# exactly, will be approximated by floating point numbers.
#
# The function jordansymbolic computes the Jordan normal form J of
# a matrix A, the transformation matrix P and its inverse P^(-1).
# Here symbolic names are used for the zeroes of the characteristic
# polynomial p not in K. Also a list of irreducible factors of p is returned.
# Specifically:
# - jordansymbolic(A) or jordansymbolic(A,K) will return [J,l], where J is
#   the Jordan normal form of A (using symbolic names if necessary) and
#   l=[ll,x], where x is a name and ll is a list of irreducible factors of
#   p(x). If symbolic names are used then xij is a zero of ll[i].
# - jordansymbolic(A,'P') or jordansymbolic(A,K,'P') will do the same as
#   jordansymbolic(A) (resp. jordansymbolic(A,K)), but now the transformation
#    matrix is assigned to P.
# - jordansymbolic(A,'P','Pinv') or jordansymbolic(A,K,'P','Pinv')will do the
#   same as jordansymbolic(A,'P') (resp. jordansymbolic(A,K,'P')), but now
#   also the inverse of the transformation matrix is assigned to Pinv.
# Here K is a set of RootOf's and/or radicals defining an algebraic extension
# of Q(the rational numbers).
#
# The function jordan computes the jordan normal form J of a matrix A with
# entries in some algebraic extension of Q, the transformation matrix P and
# its inverse P^(-1).
# Here A is considered as a matrix with complex number entries. The zeroes
# of the characteristic polynomial p are computed exactly, if possible.
# Otherwise they are approximated by floating point numbers.
# Specifically:
# - jordan(A) or jordan(A,K) will return the Jordan normal form J of A.
# - jordan(A,'P') or jordan(A,K,'P') will do the same as jordan(A) (resp.
#   jordan(A,K)), but now the transformation matrix is assigned to P.
# - jordan(A,'P','Pinv') or jordan(A,K,'P','Pinv') will do the same as
#   jordan(A,'P') (resp. jordan(A,K,'P')), but now also the inverse of the
#   transformation matrix is assigned to Pinv.
# Here K is a set of RootOf's and/or radicals defining an algebraic extension
# of Q(the rational numbers).
#
# Global description of the algorithm:
# For a given n by n matrix A over a field K, we first compute the rational
# Jordan normal form R of A. Then we compute the Jordan normal form of R,
# which is also the Jordan normal form of A.
# First consider the case where R=C(p), the companion matrix of the monic,
# irreducible polynomial p=x^n+p(n-1)*x^(n-1)+..+p1*x+p0.
# If y is a zero of p then
# (y^(n-1)+p(n-1)*y^(n-2)+..+p2*y+p1,y^(n-2)+p(n-1)*y^(n-3)+..+p3*y+p2,..
#  ..,y^2+p(n-1)*y+p(n-2),y+p(n-1),1)
# is an eigenvector of R with eigenvalue y.
# Let v1     = x^(n-1)+p(n-1)*x^(n-2)+..+p2*x+p1,
#     v2     = x^(n-2)+p(n-1)*x^(n-3)+..+p3*x+p2,
#     ...
#     v(n-2) = x^2+P(n-1)*x+p(n-2),
#     v(n-1) = x+p(n-1),
#     vn     = 1. 
# If y1,..,yn are the different zeroes of p in a splitting field of p over
# K (we asssume that p is separable, this is always true if K is a perfect
# field) we get:
#       inverse(V)*R*V=diag(y1,..,yn),
# where
#          [ v1(y1) v1(y2) ... v1(yn) ]
#          [ v2(y1) v2(y2) ... v2(yn) ]
#      V = [  ...    ...   ...  ...   ]
#          [  ...    ...   ...  ...   ]
#          [ vn(y1) vn(y2) ... vn(yn) ]
# One can prove that
#      [1 y1 ... y1^(n-1)] [v1(y1) v1(y2) ... v1(yn)] 
#      [1 y2 ... y2^(n-1)] [v2(y1) v2(y2) ... v2(yn)] 
#      [.................] [........................] =
#      [.................] [........................] 
#      [1 yn ... yn^(n-1)] [vn(y1) vn(y2) ... vn(yn)] 
#
#    = diag(diff(p,x)(y1),diff(p,x)(y2),...,diff(p,x)(yn)).
# If s and t are such that s*p+t*diff(p,x)=1 then we get
#                                            [1 y1 ... y1^(n-1)]
#                                            [1 y2 ... y2^(n-1)]
#     inverse(V)=diag(t(y1),t(y2),...,t(yn))*[.................]
#                                            [.................]
#                                            [1 yn ... yn^(n-1)]
# Let Y=diag(y1,..,yn). From V^(-1)*R*V=Y it follows that
#                          [C(p)  I             ]
#                          [    C(p)  I         ]
#   diag(V^(-1),..,V^(-1))*[          .   .     ]*diag(V,..,V)=
#                          [            C(p)  I ]
#                          [                C(p)]
#
#          [ Y I       ]
#          [   Y I     ]
#        = [     . .   ]
#          [       Y I ]
#          [         Y ]
# It is now easy to see that to get our general result, we only have to
# permute diag(V,..,V) and diag(V^(-1),..,V^(-1)).


jordansymbolic:=proc(A)
local AA,n,i,j;

  if not type(A,'matrix') then
    AA:=evalm(A)
  else
    AA:=A
  fi;
  if not type(AA,'matrix'('anything','square')) then
    ERROR(`expecting a square matrix`)
  fi;

  n:=linalg[rowdim](AA);
  for i to n do
    for j to n do
      if type(AA[i,j],indexed) then
        ERROR(`Unassigned array elements`)
      fi
    od
  od;

  if nargs>1 and type(args[2],set) then
    if args[2]={I} then
      SIMPLIFY:=simplcomplex;
      GCDEX:=gcdexgeneral;
      MULTIPLE:=multiplegeneral;
      jordansymbolicform(AA,args[2..nargs])
    else
      SIMPLIFY:=simplalgebraic;
      GCDEX:=gcdexgeneral;
      MULTIPLE:=multiplegeneral;
      jordansymbolicform(AA,args[2..nargs])
    fi
  else
    if type(AA,'matrix'('rational')) then
      SIMPLIFY:=simplrational;
      GCDEX:=gcdex;
      MULTIPLE:=lcm;
      jordansymbolicform(AA,{},args[2..nargs])
    else
      SIMPLIFY:=simplratfunc;
      GCDEX:=gcdexgeneral;
      MULTIPLE:=multiplegeneral;
      jordansymbolicform(AA,{},args[2..nargs])
    fi
  fi

end:

`normform/jordansymbolicform`:=proc(A,K,P,Pinv)
local l,R,T,Tinv,S,Sinv;

  if nargs=2 then
    R:=ratjordanform(A,K);
    l:=ratjordan_to_jordan(R)
  elif nargs=3 then
    R:=ratjordanform(A,K,'T');
    l:=ratjordan_to_jordan(R,'S');
    P:=map(SIMPLIFY,evalm(T&*S))
  else
    R:=ratjordanform(A,K,'T','Tinv');
    l:=ratjordan_to_jordan(R,'S','Sinv');
    P:=map(SIMPLIFY,evalm(T&*S));
    Pinv:=map(SIMPLIFY,evalm(Sinv&*Tinv))
  fi;

  [invariant_to_jordan(l[1]),l[2]]

end:


`normform/ratjordan_to_jordan`:=proc(R,S,Sinv)
local prim_inv,x,i,j,k,d,N,T,Tinv,Tinvlist,Tlist,exp_list,invariant,n,p,
      partT,partTinv,s,t,v,w;

  prim_inv:=ratjordan_to_priminv(R,x);

  invariant:=[];
  if nargs>=2 then
    Tlist:=[]
  fi;
  if nargs=3 then
    Tinvlist:=[]
  fi;

  N:=nops(prim_inv);
  for i to N do
    p:=prim_inv[i][1];
    exp_list:=prim_inv[i][2];
    d:=degree(p,x);
    if d=1 then
      invariant:=[op(invariant),[-coeff(p,x,0),exp_list]]
    else
      for j to d do
        invariant:=[op(invariant),[evaln(x.i.j),exp_list]]
      od
    fi;

    if nargs>=2 then
      # Compute eigenvector of C(p) with eigenvalue x
      v:=array(1..d);
      v[d]:=1;
      for j from d-1 by -1 to 1 do
        v[j]:=sum('coeff(p,x,k)*x^(k-j)','k'=j..(d-1))+x^(d-j)
      od;

      n:=sum('exp_list[j]','j'=1..nops(exp_list));

      partT:=zero_matrix(n*d,n);
      for j to n do
        for k to d do
          partT[(j-1)*d+k,j]:=v[k]
        od
      od;

      T:=array(1..n*d,1..n*d);
      if d=1 then
        linalg[copyinto](subs(x=-coeff(p,x,0),op(partT)),T,1,1)
      else
        for j to d do
          linalg[copyinto](subs(x=evaln(x.i.j),op(partT)),T,1,(j-1)*n+1)
        od
      fi;

      Tlist:=[op(Tlist),op(T)]
    fi;

    if nargs=3 then
      GCDEX(p,diff(p,x),x,'s','t');
      w:=array(1..d);
      w[1]:=SIMPLIFY(t,x);
      for j from 2 to d do
        w[j]:=SIMPLIFY(rem(x*w[j-1],p,x),x)
      od;

      partTinv:=zero_matrix(n,n*d);
      for j to n do
        for k to d do
          partTinv[j,(j-1)*d+k]:=w[k]
        od
      od;
      Tinv:=array(1..n*d,1..n*d);
      if d=1 then
        linalg[copyinto](subs(x=-coeff(p,x,0),op(partTinv)),Tinv,1,1)
      else
        for j to d do
          linalg[copyinto](subs(x=evaln(x.i.j),op(partTinv)),Tinv,(j-1)*n+1,1)
        od
      fi;
      Tinvlist:=[op(Tinvlist),op(Tinv)]
    fi
  od;

  if nargs>=2 then
    S:=linalg[diag](op(Tlist))
  fi;
  if nargs=3 then
    Sinv:=linalg[diag](op(Tinvlist))
  fi;

  [invariant,[[seq(prim_inv[i][1],i=1..N)],x]]

end:


# ratjordan_to_priminv(R,x) computes the primary invariant of a matrix
# R which is in rational Jordan normal form

`normform/ratjordan_to_priminv`:=proc(R,x)
local p,r,n,plist,exp_list,l,i,N,prim_inv;
  n:=linalg[rowdim](R);
  r:=1;
  plist:=[];
  while r<=n do
    l:=find_ratjblock(R,r,x);
    plist:=[op(plist),l];
    r:=r+l[2]*degree(l[1],x)
  od;
  p:=plist[1][1];
  exp_list:=[plist[1][2]];
  prim_inv:=[];
  N:=nops(plist);
  i:=2;
  while i<=N do
    if plist[i][1]=p then
      exp_list:=[op(exp_list),plist[i][2]]
    else
      prim_inv:=[op(prim_inv),[p,exp_list]];
      p:=plist[i][1];
      exp_list:=[plist[i][2]]
    fi;
    i:=i+1
  od;
  prim_inv:=[op(prim_inv),[p,exp_list]];
  prim_inv
end:

`normform/find_ratjblock`:=proc(R,r,x)
local i,n,e,p;
  n:=linalg[rowdim](R);
  p:=find_companion(R,r,x);
  e:=1;
  i:=r+degree(p,x);
  do
    if i>n then RETURN([p,e]) fi;
    if identitymatrix(R,i-degree(p,x),i,degree(p,x)) then
      e:=e+1;
      i:=i+degree(p,x)
    else
      RETURN([p,e])
    fi
  od
end:

`normform/find_companion`:=proc(A,r,x)
local i,j,n,p;
  n:=linalg[rowdim](A);
  i:=r+1;
  while i<=n and A[i,i-1]=1 do i:=i+1 od;
  p:=0;
  for j from r to i-1 do p:=p-A[j,i-1]*x^(j-r) od;
  p:=p+x^(i-r)
end:

`normform/identitymatrix`:=proc(A,i,j,m)
local n;
  n:=linalg[rowdim](A);
  if i+m-1>n or j+m-1>n then
    false
  else
    linalg[equal](linalg[submatrix](A,i..i+m-1,j..j+m-1),array(1..m,1..m,identity))
  fi
end:

`normform/invariant_to_jordan`:=proc(invariant)
local block_list,N,M,i,j;
  N:=nops(invariant);
  block_list:=[];
  for i to N do
    M:=nops(invariant[i][2]);
    for j to M do
      block_list:=[op(block_list),linalg[JordanBlock](invariant[i][1],invariant[i][2][j])]
    od
  od;
  linalg[diag](op(block_list))
end:


# jordan(A) computes the Jordan normal form of a matrix A with entries in
# some algebraic extension of Q. First jordansymbolic is applied to A, then
# the symbolic zeroes of the characteristic polynomial are replaced by the
# actual zeroes. The zeroes of the characteristic polynomial of A are computed
# exactly if possible. The zeroes which cannot be computed exactly are
# approximated by floating point numbers.

jordan:=proc(A)
local AA,n,i,j,l;

  if not type(A,'matrix') then
    AA:=evalm(A)
  else
    AA:=A
  fi;
  if not type(AA,'matrix'('anything','square')) then
    ERROR(`expecting a square matrix`)
  fi;

  n:=linalg[rowdim](AA);
  for i to n do
    for j to n do
      if type(AA[i,j],indexed) then
        ERROR(`Unassigned array elements`)
      fi
    od
  od;

  if nargs>1 and type(args[2],set) then
    if args[2] union {sqrt(-1),I}={sqrt(-1),I} then
      SIMPLIFY:=simplcomplex;
      GCDEX:=gcdexgeneral;
      MULTIPLE:=multiplegeneral;
      l:=jordansymbolicform(AA,args[2..nargs]);
      jordanform(l,args[3..nargs])
    else
      SIMPLIFY:=simplalgebraic;
      GCDEX:=gcdexgeneral;
      MULTIPLE:=multiplegeneral;
      l:=jordansymbolicform(AA,args[2..nargs]);
      jordanform(l,args[3..nargs])
    fi
  else
    SIMPLIFY:=simplrational;
    GCDEX:=gcdex;
    MULTIPLE:=lcm;
    l:=jordansymbolicform(AA,{},args[2..nargs]);
    jordanform(l,args[2..nargs])
  fi

end:

`normform/jordanform`:=proc(l,P,Pinv)
local N,J,x,d,z,zeroes,i,j;

  N:=nops(l[2][1]);
  x:=l[2][2];
  J:=l[1];
  for i to N do
    d:=degree(l[2][1][i],x);
    if d>1 then

      # determine zeroes
      z:=[solve(l[2][1][i]=0,x)];
      zeroes:=[];
      for j to nops(z) do
        if type(z[j],RootOf) then
          zeroes:=[op(zeroes),fsolve(op(z[j]),op(indets(op(z[j]))),complex)]
        else
          zeroes:=[op(zeroes),z[j]]
        fi
      od;

      # substitute zeroes for symbolic names
      for j to nops(zeroes) do
        J:=subs(evaln(x.i.j)=zeroes[j],op(J))
      od;
      if nargs>=2 then
        for j to nops(zeroes) do
          P:=subs(evaln(x.i.j)=zeroes[j],op(P))
        od
      fi;
      if nargs=3 then
        for j to nops(zeroes) do
          Pinv:=subs(evaln(x.i.j)=zeroes[j],op(Pinv))
        od
      fi

    fi
  od;

  op(J)

end:


`help/text/jordansymbolic` := TEXT(
`FUNCTION: jordansymbolic - compute the Jordan normal form of a matrix`,
`   `,
`CALLING SEQUENCE:`,
`   jordansymbolic(A) or jordansymbolic(A, K)`,
`   jordansymbolic(A, 'P') or jordansymbolic(A, K, 'P')`,
`   jordansymbolic(A, 'P', 'Pinv') or jordansymbolic(A, K, 'P', 'Pinv')`,
`   `,
`PARAMETERS:`,
`   A          - a square matrix`,
`   K          - an algebraic extension`,
`   'P','Pinv' - (optional) assigned the transformation matrix and its inverse`,
`   `,
`SYNOPSIS:`,
`- The function jordansymbolic(A) computes and returns the Jordan normal`,
`  form J of a matrix A.`,
`   `,
`- J has the following structure: J=diag(J11,J12,..,J21,J22,..) where the`,
`  Jij's have the following shape:`,
`   `,
`           [ xi  1              ]`,
`           [                    ]`,
`           [     xi  1          ]`,
`           [                    ]`,
`           [         .   .      ]`,
`           [                    ]`,
`           [             xi  1  ]`,
`           [                    ]`,
`           [                 xi ]`,
`   `,
`  where there are eij times xi along the diagonal. Here xi is a zero of`,
`  the characteristic polynomial p of A. If p does not split completely,`,
`  symbolic names are chosen for the missing zeroes of p. If, by some`,
`  means, one knows such missing zeroes they can be substituted for the`,
`  symbolic names. For this jordansymbolic actually returns a list [J,l],`,
`  where J is the Jordan normal form of A (using symbolic names if necessary)`,
`  and l=[ll,x], where x is a name and ll is a list of irreducible factors of`,
`  p(x). If symbolic names are used then xij is a zero of ll[i].`,
`  Convention: for each i, j->eij is non_decreasing.`,
`   `,
`- If called in the form jordansymbolic(A,'P'), then P will be assigned the`,
`  transformation matrix corresponding to the Jordan normal form,`,
`  that is, the matrix P such that inverse(P) * A * P = J.`,
`  If called in the form jordansymbolic(A,'P','Pinv'), then Pinv will be`,
`  assigned the inverse of P.`,
`   `,
`- If the optional parameter K is present, all calculations will be performed`,
`  in the algebraic number field defined by K. Here K is a set of RootOf's`,
`  and/or radicals`,
`   `,
`- When K is not present also rational functions in several variables are`,
`  allowed as matrix entries`,
`   `,
`EXAMPLES:`,
`> A := array([[-9,21,-15,4,2,0],[-10,21,-14,4,2,0],[-8,16,-11,4,2,0],`,
`>             [-6,12,-9,3,3,0],[-4,8,-6,0,5,0],[-2,4,-3,0,1,3]]);`,
`                              [  -9  21  -15  4  2  0 ]`,
`                              [                       ]`,
`                              [ -10  21  -14  4  2  0 ]`,
`                              [                       ]`,
`                              [  -8  16  -11  4  2  0 ]`,
`                         A := [                       ]`,
`                              [  -6  12   -9  3  3  0 ]`,
`                              [                       ]`,
`                              [  -4   8   -6  0  5  0 ]`,
`                              [                       ]`,
`                              [  -2   4   -3  0  1  3 ]`,
`   `,
`> l:=jordansymbolic(A,'P','Pinv');`,
`           [ 3  0  0  0   0    0  ]`,
`           [                      ]`,
`           [ 0  3  0  0   0    0  ]`,
`           [                      ]`,
`           [ 0  0  1  1   0    0  ]                                 2`,
`     l := [[                      ], [[- 3 + x, - 1 + x, 5 - 4 x + x ], x]]`,
`           [ 0  0  0  1   0    0  ]`,
`           [                      ]`,
`           [ 0  0  0  0  x31   0  ]`,
`           [                      ]`,
`           [ 0  0  0  0   0   x32 ]`,
`   `,
`> op(P);op(Pinv);`,
`             [ 3  -3/8   1   1/4   3 x31 - 17/2    3 x32 - 17/2  ]`,
`             [                                                   ]`,
`             [ 3  -3/8   1   1/4  5/2 x31 - 15/2  5/2 x32 - 15/2 ]`,
`             [                                                   ]`,
`             [ 3  -3/8   1   1/4     2 x31 - 6       2 x32 - 6   ]`,
`             [                                                   ]`,
`             [ 3  -3/8  3/4  3/8   3/2 x31 - 9/2   3/2 x32 - 9/2 ]`,
`             [                                                   ]`,
`             [ 3  -3/8  1/2  1/4      x31 - 3         x32 - 3    ]`,
`             [                                                   ]`,
`             [ 2  -1/8  1/4  1/8   1/2 x31 - 3/2   1/2 x32 - 3/2 ]`,
`   `,
`                     [    0        0      0  -1/3   0  1 ]`,
`                     [                                   ]`,
`                     [    0        0      0   8/3  -8  8 ]`,
`                     [                                   ]`,
`                     [    0        -4     6    0   -2  0 ]`,
`                     [                                   ]`,
`                     [    0        0     -4    8   -4  0 ]`,
`                     [                                   ]`,
`                     [ 3 - x31  x31 - 4   1    0    0  0 ]`,
`                     [                                   ]`,
`                     [ 3 - x32  x32 - 4   1    0    0  0 ]`,
`   `,
`> solve(x^2-4*x+5);`,
`                                  2 + I, 2 - I`,
`   `,
`> subs({x31=2+I,x32=2-I},l[1]);`,
`                          [ 3  0  0  0    0      0   ]`,
`                          [                          ]`,
`                          [ 0  3  0  0    0      0   ]`,
`                          [                          ]`,
`                          [ 0  0  1  1    0      0   ]`,
`                          [                          ]`,
`                          [ 0  0  0  1    0      0   ]`,
`                          [                          ]`,
`                          [ 0  0  0  0  2 + I    0   ]`,
`                          [                          ]`,
`                          [ 0  0  0  0    0    2 - I ]`,
`   `,
`> subs({x31=2+I,x32=2-I},op(P));subs({x31=2+I,x32=2-I},op(Pinv));`,
`              [ 3  -3/8   1   1/4   - 5/2 + 3 I    - 5/2 - 3 I  ]`,
`              [                                                 ]`,
`              [ 3  -3/8   1   1/4  - 5/2 + 5/2 I  - 5/2 - 5/2 I ]`,
`              [                                                 ]`,
`              [ 3  -3/8   1   1/4    - 2 + 2 I      - 2 - 2 I   ]`,
`              [                                                 ]`,
`              [ 3  -3/8  3/4  3/8  - 3/2 + 3/2 I  - 3/2 - 3/2 I ]`,
`              [                                                 ]`,
`              [ 3  -3/8  1/2  1/4     - 1 + I        - 1 - I    ]`,
`              [                                                 ]`,
`              [ 2  -1/8  1/4  1/8  - 1/2 + 1/2 I  - 1/2 - 1/2 I ]`,
`   `,
`                      [   0       0      0  -1/3   0  1 ]`,
`                      [                                 ]`,
`                      [   0       0      0   8/3  -8  8 ]`,
`                      [                                 ]`,
`                      [   0       -4     6    0   -2  0 ]`,
`                      [                                 ]`,
`                      [   0       0     -4    8   -4  0 ]`,
`                      [                                 ]`,
`                      [ 1 - I  - 2 + I   1    0    0  0 ]`,
`                      [                                 ]`,
`                      [ 1 + I  - 2 - I   1    0    0  0 ]`,
`   `,
`> A := array([[-3-I,1,2+I,7-9*I],`,
`              [-2,1,1,5-I],`,
`              [-2-2*I,1,2+2*I,4-2*I],`,
`              [2,0,-1,-2+8*I]]);`,
`                        [  - 3 - I   1   2 + I    7 - 9 I  ]`,
`                        [                                  ]`,
`                        [     -2     1     1       5 - I   ]`,
`                   A := [                                  ]`,
`                        [ - 2 - 2 I  1  2 + 2 I   4 - 2 I  ]`,
`                        [                                  ]`,
`                        [     2      0     -1    - 2 + 8 I ]`,
`   `,
`> jordansymbolic(A,{I});`,
`  [ 1 + I    0     0    0  ]`,
`  [                        ]`,
`  [   0    1 + I   0    0  ]                                            2`,
` [[                        ], [[- 1 - I + x, 2 + 5 I - (- 4 + 7 I) x + x ], x]]`,
`  [   0      0    x21   0  ]`,
`  [                        ]`,
`  [   0      0     0   x22 ]`,
`   `,
`> s:=sqrt(2):`,
`> A := array([[s,1-3*s],[3,1/s]]);`,
`                                [  1/2         1/2 ]`,
`                                [ 2     1 - 3 2    ]`,
`                           A := [                  ]`,
`                                [             1/2  ]`,
`                                [   3    1/2 2     ]`,
`   `,
`> jordansymbolic(A,{sqrt(2)});`,
`              [ x11   0  ]             1/2        1/2      2`,
`             [[          ], [[- 2 + 9 2    - 3/2 2    x + x ], x]]`,
`              [  0   x12 ]`,
`> alias(a=RootOf(X^3-2*X+X-5)):`,
`> A := array([[1-a,2+a^2],[3+a-2*a^2,3]]);`,
`                              [                    2 ]`,
`                              [     1 - a     2 + a  ]`,
`                         A := [                      ]`,
`                              [            2         ]`,
`                              [ 3 + a - 2 a      3   ]`,
`   `,
`> jordansymbolic(A,{a});`,
`             [ x11   0  ]             2                      2`,
`            [[          ], [[- 8 + 3 a  + 4 a - (4 - a) x + x ], x]]`,
`             [  0   x12 ]`,
`> A:=array([[-1,-1/y],[y^2+y+1,y+1]]);`,
`                                [     -1      - 1/y ]`,
`                                [                   ]`,
`                           A := [  2                ]`,
`                                [ y  + y + 1  y + 1 ]`,
`   `,
`> l:=jordansymbolic(A);`,
`                         [ x11   0  ]                 2`,
`                   l := [[          ], [[1/y - y x + x ], x]]`,
`                         [  0   x12 ]`,
`   `,
`> x:=l[2][2]:`,
`> z:=solve(x^2-y*x+1/y,x);`,
`                                    3 1/2                      3 1/2`,
`                            (- 4 + y )                 (- 4 + y )`,
`           z := 1/2 y + 1/2 -------------, 1/2 y - 1/2 -------------`,
`                                  1/2                        1/2`,
`                                 y                          y`,
`   `,
`> map(normal,subs({x11=z[1],x12=z[2]},l[1]));`,
`             [      3/2           3 1/2                           ]`,
`             [     y    + (- 4 + y )                              ]`,
`             [ 1/2 --------------------              0            ]`,
`             [              1/2                                   ]`,
`             [             y                                      ]`,
`             [                                                    ]`,
`             [                                3/2           3 1/2 ]`,
`             [                               y    - (- 4 + y )    ]`,
`             [             0             1/2 -------------------- ]`,
`             [                                        1/2         ]`,
`             [                                       y            ]`,
`   `,
`SEE ALSO: smithex, ismithex, frobenius, ratjordan, jordan,`,
`          Frobenius, Ratjordan, Jordansymbolic`
):


`help/text/jordan` := TEXT(
`FUNCTION: jordan - compute the Jordan normal form of a matrix`,
`   `,
`CALLING SEQUENCE:`,
`   jordan(A) or jordan(A, K)`,
`   jordan(A, 'P') or jordan(A, K, 'P')`,
`   jordan(A, 'P', 'Pinv') or jordan(A, K, 'P', 'Pinv')`,
`   `,
`PARAMETERS:`,
`   A          - a square matrix`,
`   K          - an algebraic extension`,
`   'P','Pinv' - (optional) assigned the transformation matrix and its inverse`,
`   `,
`SYNOPSIS:`,
`- The function jordan(A) computes and returns the Jordan normal`,
`  form J of a matrix A with entries in an algebraic extension of Q (the`,
`  rational numbers).`,
`   `,
`- J has the following structure: J=diag(J11,J12,..,J21,J22,..) where the`,
`  Jij's have the following shape:`,
`   `,
`           [ xi  1              ]`,
`           [                    ]`,
`           [     xi  1          ]`,
`           [                    ]`,
`           [         .   .      ]`,
`           [                    ]`,
`           [             xi  1  ]`,
`           [                    ]`,
`           [                 xi ]`,
`   `,
`  where there are eij times xi along the diagonal. Here xi is a zero of`,
`  the characteristic polynomial p of A. The zeroes of the characteristic`,
`  polynomial are computed exactly, if possible. Otherwise they are`,
`  approximated by floating point numbers.`,
`  Convention: for each i, j->eij is non_decreasing.`,
`   `,
`- If called in the form jordan(A,'P'), then P will be assigned the`,
`  transformation matrix corresponding to the Jordan normal form,`,
`  that is, the matrix P such that inverse(P) * A * P = J.`,
`  If called in the form jordan(A,'P','Pinv'), then Pinv will be`,
`  assigned the inverse of P.`,
`   `,
`- If the optional parameter K is present, all calculations will be performed`,
`  in the algebraic number field defined by K. Here K is a set of RootOf's`,
`  and/or radicals`,
`   `,
`EXAMPLES:`,
`> A := array([[-9,21,-15,4,2,0],[-10,21,-14,4,2,0],[-8,16,-11,4,2,0],`,
`>             [-6,12,-9,3,3,0],[-4,8,-6,0,5,0],[-2,4,-3,0,1,3]]);`,
`                              [  -9  21  -15  4  2  0 ]`,
`                              [                       ]`,
`                              [ -10  21  -14  4  2  0 ]`,
`                              [                       ]`,
`                              [  -8  16  -11  4  2  0 ]`,
`                         A := [                       ]`,
`                              [  -6  12   -9  3  3  0 ]`,
`                              [                       ]`,
`                              [  -4   8   -6  0  5  0 ]`,
`                              [                       ]`,
`                              [  -2   4   -3  0  1  3 ]`,
`   `,
`> jordan(A,'P','Pinv');`,
`                          [ 1  1  0  0    0      0   ]`,
`                          [                          ]`,
`                          [ 0  1  0  0    0      0   ]`,
`                          [                          ]`,
`                          [ 0  0  3  0    0      0   ]`,
`                          [                          ]`,
`                          [ 0  0  0  3    0      0   ]`,
`                          [                          ]`,
`                          [ 0  0  0  0  2 + I    0   ]`,
`                          [                          ]`,
`                          [ 0  0  0  0    0    2 - I ]`,
`   `,
`> op(P);op(Pinv);`,
`              [  1   1/4  3  -3/8   - 5/2 + 3 I    - 5/2 - 3 I  ]`,
`              [                                                 ]`,
`              [  1   1/4  3  -3/8  - 5/2 + 5/2 I  - 5/2 - 5/2 I ]`,
`              [                                                 ]`,
`              [  1   1/4  3  -3/8    - 2 + 2 I      - 2 - 2 I   ]`,
`              [                                                 ]`,
`              [ 3/4  3/8  3  -3/8  - 3/2 + 3/2 I  - 3/2 - 3/2 I ]`,
`              [                                                 ]`,
`              [ 1/2  1/4  3  -3/8     - 1 + I        - 1 - I    ]`,
`              [                                                 ]`,
`              [ 1/4  1/8  2  -1/8  - 1/2 + 1/2 I  - 1/2 - 1/2 I ]`,
`   `,
`                      [   0       -4     6    0   -2  0 ]`,
`                      [                                 ]`,
`                      [   0       0     -4    8   -4  0 ]`,
`                      [                                 ]`,
`                      [   0       0      0  -1/3   0  1 ]`,
`                      [                                 ]`,
`                      [   0       0      0   8/3  -8  8 ]`,
`                      [                                 ]`,
`                      [ 1 - I  - 2 + I   1    0    0  0 ]`,
`                      [                                 ]`,
`                      [ 1 + I  - 2 - I   1    0    0  0 ]`,
`   `,
`> A := array([[-3-I,1,2+I,7-9*I],`,
`              [-2,1,1,5-I],`,
`              [-2-2*I,1,2+2*I,4-2*I],`,
`              [2,0,-1,-2+8*I]]);`,
`                        [  - 3 - I   1   2 + I    7 - 9 I  ]`,
`                        [                                  ]`,
`                        [     -2     1     1       5 - I   ]`,
`                   A := [                                  ]`,
`                        [ - 2 - 2 I  1  2 + 2 I   4 - 2 I  ]`,
`                        [                                  ]`,
`                        [     2      0     -1    - 2 + 8 I ]`,
`   `,
`> jordan(A,{I});`,
`                               [1 + I, 0, 0, 0]`,
`   `,
`                               [0, 1 + I, 0, 0]`,
`   `,
`                                                       1/2`,
`                 [0, 0, - 2 + 7/2 I + 1/2 (- 41 - 76 I)   , 0]`,
`   `,
`                                                          1/2`,
`                 [0, 0, 0, - 2 + 7/2 I - 1/2 (- 41 - 76 I)   ]`,
`   `,
`> s:=sqrt(2):`,
`> A := array([[s,1-3*s],[3,1/s]]);`,
`                                [  1/2         1/2 ]`,
`                                [ 2     1 - 3 2    ]`,
`                           A := [                  ]`,
`                                [             1/2  ]`,
`                                [   3    1/2 2     ]`,
`   `,
`> jordan(A,{sqrt(2)});`,
`                         1/2                 1/2 1/2  1/2`,
`                   [3/4 2    + 1/4 (25 - 72 2   )    2   , 0]`,
`   `,
`                            1/2                 1/2 1/2  1/2`,
`                   [0, 3/4 2    - 1/4 (25 - 72 2   )    2   ]`,
`   `,
`> alias(a=RootOf(X^3-2*X+X-5)):`,
`> A := array([[1-a,2+a^2],[3+a-2*a^2,3]]);`,
`                              [                    2 ]`,
`                              [     1 - a     2 + a  ]`,
`                         A := [                      ]`,
`                              [            2         ]`,
`                              [ 3 + a - 2 a      3   ]`,
`   `,
`> jordan(A,{a});`,
`                                                    2 1/2`,
`                  [2 - 1/2 a + 1/2 (48 - 24 a - 11 a )   , 0]`,
`   `,
`                                                       2 1/2`,
`                  [0, 2 - 1/2 a - 1/2 (48 - 24 a - 11 a )   ]`,
`   `,
`> A := array([[-12752,-6285,-9457,-7065,-4939,-5865,-3769],`,
`              [13028,6430,9656,7213,5041,5984,3841],`,
`              [16425,8080,12192,9108,6370,7569,4871],`,
`              [-6065,-2979,-4508,-3364,-2354,-2801,-1803],`,
`              [2968,1424,2231,1664,1171,1404,919],`,
`              [-22762,-11189,-16902,-12627,-8833,-10498,-6760],`,
`              [23112,11400,17135,12799,8946,10622,6821]]);`,
`              [ -12752   -6285   -9457   -7065  -4939   -5865  -3769 ]`,
`              [                                                      ]`,
`              [  13028   6430    9656    7213    5041   5984    3841 ]`,
`              [                                                      ]`,
`              [  16425   8080    12192   9108    6370   7569    4871 ]`,
`              [                                                      ]`,
`         A := [  -6065   -2979   -4508   -3364  -2354   -2801  -1803 ]`,
`              [                                                      ]`,
`              [  2968    1424    2231    1664    1171   1404    919  ]`,
`              [                                                      ]`,
`              [ -22762  -11189  -16902  -12627  -8833  -10498  -6760 ]`,
`              [                                                      ]`,
`              [  23112   11400   17135   12799   8946   10622   6821 ]`,
`   `,
`> jordan(A);`,
`                             1/2`,
`                           [2   , 0, 0, 0, 0, 0, 0]`,
`   `,
`                                 1/2`,
`                          [0, - 2   , 0, 0, 0, 0, 0]`,
`   `,
`                       [0, 0, -1.804919732, 0, 0, 0, 0]`,
`   `,
`                       [0, 0, 0, -1.124910946, 0, 0, 0]`,
`   `,
`                [0, 0, 0, 0, .6203192706 + 1.035886564 I, 0, 0]`,
`   `,
`                [0, 0, 0, 0, 0, .6203192706 - 1.035886564 I, 0]`,
`   `,
`                        [0, 0, 0, 0, 0, 0, 1.689192137]`,
`   `,
`SEE ALSO: smithex, ismithex, frobenius, ratjordan, jordansymbolic,`,
`          Frobenius, Ratjordan, Jordansymbolic`
):



############################################################################
############################################################################
##
##          smithex
##
###########################################################################
###########################################################################
# The MapleV algorithm linalg[smith] has been extended such that
# smithex(A,x,'L','R') returns the smith normal form S of A and
# L and R are unimodular matrices such that A = L*S*R.
# Most changes and additions are between signs '#++++++++++' and '#----------'.
# Authors of adaptation: T.M.L. Mulders, A.H.M. Levelt
#                        Mathematics Department
#                        University of Nijmegen
# E-mail: mulders@sci.kun.nl, ahml@sci.kun.nl
#
# January 1993

smithex := proc(B,x,L,R)
local a,b,g,i,j,k,l,m,n,q,r,s,t,lc,tb,temp,A,localB,Left,Right,isClear;


        option `Copyright 1990 by the University of Waterloo`;
        if not type(x,name) then ERROR(`2nd argument must be a name`) fi;
        if not type(B,'matrix') then localB:=evalm(B) else localB:=B fi;
        if not type(localB,'matrix(polynom(anything,x))') then
            ERROR(`matrix entries must be univariate polynomials in`,x) fi;
        if not type(localB,'matrix(polynom(ratpoly(rational),x))') then
            ERROR(`not implemented`) fi;
#++++++++++
        if nargs=4 and not (type(L,name) and type(R,name)) then
            ERROR(`3rd and 4th argument must be names`) fi;
#----------

        n := linalg[rowdim](localB);
        m := linalg[coldim](localB);
        A := array(1..n,1..m);
 
#++++++++++
        Left := Id(n);
        Right := Id(m);
#----------

        userinfo(1,smithex,`dimension`,n,` by`,m);
        for i to n do for j to m do A[i,j] := collect(localB[i,j],x,normal) 
        od od;

        for k to min(n,m) do

            #  Pivot selection from row k and column k
            for i from k to n while A[i,k] = 0 do od;
            for j from k to m while A[k,j] = 0 do od;
            if i > n and j > m then next fi;

            #  Select the smallest non-zero entry as the pivot
            for l from i+1 to n do
                if A[l,k] = 0 then next fi;
                if degree(A[l,k],x) < degree(A[i,k],x) then i := l fi
            od;
            for l from j+1 to m do
                if A[k,l] = 0 then next fi;
                if degree(A[k,l],x) < degree(A[k,j],x) then j := l fi
            od;

            if i <= n and (j > m or
                degree(A[i,k],x) < degree(A[k,j],x)) then
                    #  Pivot is A[i,k], interchange row k,i if necessary
                    if i <> k then
                        for l from k to m do
                            t := A[i,l]; A[i,l] := A[k,l]; A[k,l] := t
                        od;
#++++++++++
                        for l  to n do
                            t := Left[l,i]; Left[l,i] := Left[l,k]; Left[l,k] := t
                        od
#----------
                    fi
            else    #  Pivot is A[k,j], interchange column k,j if necessary
                    if j <> k then
                        for l from k to n do
                            t := A[l,j]; A[l,j] := A[l,k]; A[l,k] := t
                        od;
#++++++++++
                        for l to m do
                            t := Right[j,l]; Right[j,l] := Right[k,l]; Right[k,l] := t
                        od
#----------  
                    fi
            fi;

userinfo(2,smithex,`elimination at row`,k);
          isClear := false;
          while not isClear do

            #  0 out column k from k+1 to n
            for i from k+1 to n do
                if A[i,k] = 0 then next fi;
                g := gcdex(A[k,k], A[i,k], x, 's', 't');
                a := quo(A[k,k],g,x); b := quo(A[i,k],g,x);
                #
                #  We have  s A[k,k]/g + t A[i,k]/g = 1
                #
                #       [  s  t ]  [ A[k,k]  A[k,j] ]   [ g  ... ]
                #       [       ]  [                ] = [        ]
                #       [ -b  a ]  [ A[i,k]  A[i,j] ]   [ 0  ... ]
                #
                #       for j = k+1..m  where note  s a + t b = 1
                #
                for j from k+1 to m do
                    temp := normal( s*A[k,j] + t*A[i,j] );
                    A[i,j] := normal( a*A[i,j] - b*A[k,j] );
                    A[k,j] := temp
                od;
#++++++++++
                for j to n do
                    temp := normal(a*Left[j,k] + b*Left[j,i]);
                    Left[j,i] := normal(-t*Left[j,k] + s*Left[j,i]);
                    Left[j,k] := temp
                od;
#----------
                A[k,k] := g;
                A[i,k] := 0
            od;
            isClear := true;

            #  0 out row k from k+1 to m
#++++++++++
            for i from k+1 to m do 
                A[k,i] := rem(A[k,i],A[k,k],x,'q'); 
                for j to m do Right[k,j] := normal(Right[k,j] + q* Right[i,j]) od
            od;
#----------
            for i from k+1 to m do
                if A[k,i] = 0 then next fi;
                g := gcdex(A[k,k], A[k,i], x, 's', 't');
                a := quo(A[k,k],g,x); b := quo(A[k,i],g,x);
                for j from k+1 to n do
                    temp := normal( s*A[j,k] + t*A[j,i] );
                    A[j,i] := normal( a*A[j,i] - b*A[j,k] );
                    A[j,k] := temp
                od;
#++++++++++
                for j to m do
                    temp := normal( a*Right[k,j] + b*Right[i,j]);
                    Right[i,j] := normal(-t*Right[k,j] + s*Right[i,j]);
                    Right[k,j] := temp
                od;
#----------
                A[k,k] := g;
                A[k,i] := 0;
                isClear := false;
            od;

          od;

        od;
        r := 0;
        #  At this point, A is diagonal: some A[i,i] may be zero
        #  Move non-zero's up also making all entries unit normal
        for i to min(n,m) do
            if A[i,i] <> 0 then
                r := r+1;
#++++++++++
                lc := lcoeff(A[i,i],x);
                A[r,r] := normal(A[i,i]/lc);
                if i=r then 
                    for j to m do Right[i,j] := normal(Right[i,j]*lc) od
                else
                    A[i,i] := 0;
                    for j to n do 
                        temp := Left[j,r];
                        Left[j,r] := Left[j,i];
                        Left[j,i] := temp
                    od;
                    for j to m do
                        temp := normal(Right[i,j]*lc);
                        Right[i,j] := normal(Right[r,j]/lc);
                        Right[r,j] := temp
                    od
                fi
#----------
            fi
        od;
#  Now make A[i,i] | A[i+1,i+1] for 1 <= i < r
        for i to r-1 do
            for j from i+1 to r while A[i,i] <> 1 do
#++++++++++
                g := gcdex(A[i,i],A[j,j],x,'s','t');
                a := quo(A[i,i],g,x); b:= quo(A[j,j],g,x);
                A[i,i] := g;
                A[j,j] := normal( a*A[j,j] );
                for k to n do
                  temp := normal(a*Left[k,i] + b*Left[k,j]);
                  Left[k,j] := normal(-t*Left[k,i] + s*Left[k,j]);
                  Left[k,i] := temp
                od;
                for k to m do
                  tb := normal(t*b);
                  temp := normal((1-tb)*Right[i,k] + tb*Right[j,k]);
                  Right[j,k] := normal(-Right[i,k] + Right[j,k]);
                  Right[i,k] := temp
                od
#----------
            od
        od;

#++++++++++
        if nargs>2 then L := eval(Left) fi;
        if nargs>3 then R := eval(Right) fi;
#----------

        subs('localB'=localB,op(A));
        if has(",'localB') then ERROR(`undefined matrix elements`)
        else " fi;

end:


`help/text/smithex` := TEXT(
`FUNCTION: smithex - Compute the Smith normal form S of a matrix`,
`   `,
`CALLING SEQUENCE:`,
`   smithex(A, x, 'L', 'R')`,
`   `,
`PARAMETERS:`,
`   A        - a rectangular matrix of univariate polynomials in x`,
`   x        - the variable name`,
`   'L', 'R' - assigned unimodular matrices such that L*S*R=A`,
`   `,
`SYNOPSIS:`,
`- The Smith normal form of an n by m matrix with univariate polynomial entries`,
`  in x over a field F is computed.  That is, the polynomials are then regarded`,
`  as elements of the Euclidean domain F[x].`,
`   `,
`- This routine is only as powerful as Maple's normal function, i.e. at`,
`  present it only understands the field Q of rational numbers and rational`,
`  functions over Q.`,
`   `,
`- The Smith normal form is a diagonal matrix S where:`,
`    - rank(A) = number of nonzero rows (columns) of S`,
`    - S[i,i] is a monic polynomial for 0 < i <= rank(A)`,
`    - S[i,i] divides S[i+1,i+1] for 0 < i < rank(A)`,
`    - S[i,i] is the greatest common divisor of all i by i minors of A`,
`  Hence if n = m and rank(A) = n then product(S[i,i],i=1..n)=`,
`  det(A)/lcoeff(det(A),x).`,
`   `,
`EXAMPLES:`,
`> A := array([[3*x,x^2+x],[0,x^2]]);`,
`                                   [       2     ]`,
`                                   [ 3 x  x  + x ]`,
`                              A := [             ]`,
`                                   [         2   ]`,
`                                   [  0     x    ]`,
`   `,
`> smithex(A,x,'L','R');`,
`                                   [ x   0 ]`,
`                                   [       ]`,
`                                   [     2 ]`,
`                                   [ 0  x  ]`,
`   `,
`> op(L);op(R);`,
`                                    [ 1  0 ]`,
`                                    [      ]`,
`                                    [ x  1 ]`,
`   `,
`                                 [  3  x + 1 ]`,
`                                 [           ]`,
`                                 [ -3   - x  ]`,
`   `,
`> A := array([[y^2*x,x^2-(1+y)*x],[x,x^2*(y-2)]]);`,
`                              [  2     2             ]`,
`                              [ y  x  x  - (1 + y) x ]`,
`                         A := [                      ]`,
`                              [          2           ]`,
`                              [   x     x  (y - 2)   ]`,
`   `,
`> smithex(A,x,'L','R');`,
`                      [ x                0               ]`,
`                      [                                  ]`,
`                      [        3        2                ]`,
`                      [    x (y  x - 2 y  x - x + 1 + y) ]`,
`                      [ 0  ----------------------------- ]`,
`                      [             3      2             ]`,
`                      [            y  - 2 y  - 1         ]`,
`   `,
`> op(L);op(R);`,
`             [      5      4    2            3        2           ]`,
`             [   - y  + 2 y  + y  + 1 + y + y  x - 2 y  x - x     ]`,
`             [ - --------------------------------------------  -1 ]`,
`             [                    3      2                        ]`,
`             [                   y  - 2 y  - 1                    ]`,
`             [                                                    ]`,
`             [                        1                         0 ]`,
`   `,
`                      [  1           x (y - 2)          ]`,
`                      [                                 ]`,
`                      [                    3      2     ]`,
`                      [ -1  - x y + 2 x + y  - 2 y  - 1 ]`,
`   `,
`SEE ALSO:  ismithex, Smith`
):



############################################################################
############################################################################
##
##          ismithex
##
###########################################################################
###########################################################################
# The MapleV algorithm linalg[ismith] has been extended such that
# ismithex(A,'L','R') returns the smith normal form S of A and
# L and R are unimodular matrices such that A = L*S*R.
# Most changes and additions are between signs '#++++++++++' and '#------!
# Authors of adaptation: T.M.L. Mulders, A.H.M. Levelt
#                        Mathematics Department
#                        University of Nijmegen
# E-mail: mulders@sci.kun.nl, ahml@sci.kun.nl
#
# January 1993


ismithex := proc(BB,L,R)
local B,a,b,g,i,j,k,l,m,n,q,s,t,tb,temp,A,Left,Right,isClear,sgn;

        option `Copyright 1990 by the University of Waterloo`;
        if not type(BB,'matrix') then B:=evalm(BB) else B:=BB fi;
        if not type(B, 'matrix') then ERROR(`invalid arguments`) fi;
#++++++++++
        if nargs=3 and not (type(L,name) and type(R,name)) then
            ERROR(`2nd and 3rd argument must be names`) fi;
#----------
      
        n := linalg[rowdim](B);
        m := linalg[coldim](B);
userinfo(1,ismithex,`dimension`,n,'`by`',m);
        A := array(1..n,1..m);

#++++++++++
        Left := Id(n);
        Right := Id(m);
#----------

        for i to n do
            for j to m do
                if type(B[i,j],integer) then A[i,j] := B[i,j]
                else ERROR(`matrix entries must be integers`)
                fi
            od
        od;

        for k to min(n,m) do

            #  Pivot selection from row k and column k
            for i from k to n while A[i,k] = 0 do od;
            for j from k to m while A[k,j] = 0 do od;
            if i > n and j > m then next fi;

            #  Select the smallest non-zero entry as the pivot
            for l from i+1 to n do
                if A[l,k] = 0 then next fi;
                if abs(A[l,k]) < abs(A[i,k]) then i := l fi
            od;
            for l from j+1 to m do
                if A[k,l] = 0 then next fi;
                if abs(A[k,l]) < abs(A[k,j]) then j := l fi
            od;

            if i <= n and (j > m or abs(A[i,k]) < abs(A[k,j])) then
                    #  Pivot is A[i,k], interchange row k,i if necessary
                    if i <> k then
                        for l from k to m do
                            t := A[i,l]; A[i,l] := A[k,l]; A[k,l] := t
                        od;
#++++++++++
                        for l  to n do
                            t := Left[l,i]; Left[l,i] := Left[l,k]; Left[l,k] := t
                        od
#----------

                    fi
            else    #  Pivot is A[k,j], interchange column k,j if necessary
                    if j <> k then
                        for l from k to n do
                            t := A[l,j]; A[l,j] := A[l,k]; A[l,k] := t
                        od;
#++++++++++
                        for l to m do
                            t := Right[j,l]; Right[j,l] := Right[k,l]; Right[k,l] := t
                        od
#----------

                    fi
            fi;

userinfo(2,ismithex,`elimination at row`,k);

          isClear := false;
          while not isClear do

            #  Zero out column k from k+1 to n
            for i from k+1 to n do
                if A[i,k] = 0 then next fi;
                g := igcdex(A[k,k], A[i,k], 's', 't');
                a := iquo(A[k,k],g); b := iquo(A[i,k],g);
                #
                #  We have  s A[k,k]/g + t A[i,k]/g = 1
                #
                #       [  s  t ]  [ A[k,k]  A[k,j] ]   [ g  ... ]
                #       [       ]  [                ] = [        ]
                #       [ -b  a ]  [ A[i,k]  A[i,j] ]   [ 0  ... ]
                #
                #       for j = k+1..m  where note  s a + t b = 1
                #
                for j from k+1 to m do
                    temp := s*A[k,j] + t*A[i,j];
                    A[i,j] := a*A[i,j] - b*A[k,j];
                    A[k,j] := temp
                od;
#++++++++++
                for j to n do
                    temp := a*Left[j,k] + b*Left[j,i];
                    Left[j,i] := -t*Left[j,k] + s*Left[j,i];
                    Left[j,k] := temp
                od;
#----------
                A[k,k] := g;
                A[i,k] := 0
            od;
            isClear := true;

            #  Zero out row k from k+1 to m
#++++++++++
            for i from k+1 to m do
                A[k,i] := irem(A[k,i],A[k,k],'q');
                for j to m do Right[k,j] := Right[k,j] + q*Right[i,j] od
            od;
#----------
            for i from k+1 to m do
                if A[k,i] = 0 then next fi;
                g := igcdex(A[k,k], A[k,i], 's', 't');
                a := iquo(A[k,k],g); b := iquo(A[k,i],g);
                for j from k+1 to n do
                    temp := s*A[j,k] + t*A[j,i];
                    A[j,i] := a*A[j,i] - b*A[j,k];
                    A[j,k] := temp
                od;
#++++++++++
                for j to m do
                    temp:= a*Right[k,j] + b*Right[i,j];
                    Right[i,j] := -t*Right[k,j] + s*Right[i,j];
                    Right[k,j] := temp
                od;
#----------
                A[k,k] := g;
                A[k,i] := 0;
                isClear := false;
            od;

          od;

        od;


        l := 0;
        #  At this point, A is diagonal: some A[i,i] may be zero
        #  Move non-zero's up also making all entries unit normal
        for i to min(n,m) do
            if A[i,i] <> 0 then
                l := l+1;
#++++++++++
                sgn := sign(A[i,i]);
                A[l,l] := sgn*A[i,i];
                if i=l then
                    for j to m do Right[i,j] := sgn*Right[i,j] od
                else
                    A[i,i] := 0;
                    for j to n do
                        temp := Left[j,l];
                        Left[j,l] := Left[j,i];
                        Left[j,i] := temp
                    od;
                    for j to m do
                        temp := sgn*Right[i,j];
                        Right[i,j] := sgn*Right[l,j];
                        Right[l,j] := temp
                    od
                fi
#----------
            fi
        od;
        
        #  Now make A[i,i] | A[i+1,i+1] for 1 <= i < l
        for i to l-1 do
            for j from i+1 to l while A[i,i] <> 1 do
#++++++++++
                g := igcdex(A[i,i],A[j,j],'s','t');
                a := iquo(A[i,i],g); b:= iquo(A[j,j],g);
                A[i,i] := g;
                A[j,j] := a*A[j,j];
                for k to n do
                  temp := a*Left[k,i] + b*Left[k,j];
                  Left[k,j] := -t*Left[k,i] + s*Left[k,j];
                  Left[k,i] := temp
                od;
                for k to m do
                  tb := t*b;
                  temp := (1-tb)*Right[i,k] + tb*Right[j,k];
                  Right[j,k] := -Right[i,k] + Right[j,k];
                  Right[i,k] := temp
                od
#----------
            od
        od;

#++++++++++
        if nargs>1 then L := eval(Left) fi;
        if nargs>2 then R := eval(Right) fi;
#----------

        op(A)

end:


`help/text/ismithex` := TEXT(
`FUNCTION: ismithex - integer-only Smith normal form S of a matrix`,
`   `,
`CALLING SEQUENCE:`,
`   ismithex(A, 'L', 'R')`,
`   `,
`PARAMETERS:`,
`   A        - a rectangular matrix of integers`,
`   'L', 'R' - assigned unimodular matrices such that L*S*R=A`,
`   `,
`SYNOPSIS:`,
`- The function ismithex computes the Smith normal form S of an n by m`,
`  rectangular matrix of integers.`,
`   `,
`- If two n by m matrices have the same Smith normal form, they are`,
`  equivalent.`,
`   `,
`- The Smith normal form is a diagonal matrix S where:`,
`    - rank(A) = number of nonzero rows (columns) of S`,
`    - sign(S[i,i]) = 1  for 0 < i <= rank(A)`,
`    - S[i,i] divides S[i+1,i+1] for 0 < i < rank(A)`,
`    - S[i,i] is the greatest common divisor of all i by i minors of A`,
`  Hence if n = m and rank(A) = n then abs(det(A)) = product(S[i,i],i=1..n).`,
`   `,
`- The Smith normal form is obtained by doing elementary row and column opera-`,
`  tions. This includes interchanging rows (columns), multiplying through a`,
`  row (column) by -1, and adding integral multiples of one row (column) to`,
`  another.`,
`   `,
`- Although the rank and determinant can be easily obtained from S this is not`,
`  an efficient method for computing these quantities except that this may`,
`  yield a partial factorization of det(A) without doing any explicit`,
`  factorizations.`,
`   `,
`EXAMPLES:`,
`> A := array( [[9,-36,30], [-36,192,-180], [30,-180,180]] );`,
`                                 [  9    -36   30  ]`,
`                                 [                 ]`,
`                            A := [ -36   192  -180 ]`,
`                                 [                 ]`,
`                                 [  30  -180   180 ]`,
`   `,
`> ismithex(A,'L','R');`,
`                                 [ 3   0   0 ]`,
`                                 [           ]`,
`                                 [ 0  12   0 ]`,
`                                 [           ]`,
`                                 [ 0   0  60 ]`,
`   `,
`> op(L);op(R);`,
`                               [ -17   -5   -4 ]`,
`                               [               ]`,
`                               [  64   19   15 ]`,
`                               [               ]`,
`                               [ -50  -15  -12 ]`,
`   `,
`                                [  1  -24   30 ]`,
`                                [              ]`,
`                                [ -1   25  -30 ]`,
`                                [              ]`,
`                                [  0   -1   1  ]`,
`SEE ALSO:  smithex`
):

#save help,
#`normform/identitymatrix`, `normform/ratjordan_to_priminv`, 
#`normform/frobenius_to_ratjordan`, `normform/frobeniusform`, ratjordan, 
#`normform/companion_to_ratjordan`, `normform/find_companion`, `normform/Id`, 
#`normform/invfact_to_frobenius`, `normform/simplcomplex`, 
#`normform/multiplegeneral`, `normform/frobenius_to_invfact`, 
#`normform/invariant_to_jordan`, `normform/ratjordanform`, 
#`normform/zero_matrix`, `normform/plist_to_polycompanion`, smithex, 
#`help/text/smithex`, `normform/simplalgebraic`, `help/text/ratjordan`, 
#frobenius, `help/text/jordansymbolic`, `normform/inv`, ismithex, 
#`normform/cyclic_to_frobenius`, `normform/cyclic_vectors`, `normform/mysmith`, 
#`normform/deg_sort`, `normform/gcdexgeneral`, `normform/make_ratj_block`, 
#`normform/jordanform`, jordan, `normform/jordansymbolicform`, 
#`help/text/frobenius`, `normform/uppersmith`, `normform/basis`, 
#`normform/find_ratjblock`, `help/text/jordan`, `normform/ratjordan_to_jordan`, 
#`normform/priminv_to_ratjordan`, `normform/simplrational`, 
#`normform/simplratfunc`, `help/text/ismithex`, jordansymbolic,
#`normform.m`;
#quit

